Memory Tagging: A Memory Efficient Design

ARM recently introduced a security feature called Memory Tagging Extension or MTE, which is designed to defend against common memory safety vulnerabilities, such as buffer overflow and use after free. In this paper, we examine three aspects of MTE. First, we survey how modern software systems, such as Glibc, Android, Chrome, Linux, and LLVM, use MTE. We identify some common weaknesses and propose improvements. Second, we develop and experiment with an architectural improvement to MTE that improves its memory efficiency. Our design enables longer memory tags, which improves the accuracy of MTE. Finally, we discuss a number of enhancements to MTE to improve its security against certain memory safety attacks.

==> conclusion.tex <==
\section{Conclusion}

In this work, we presented an in-depth survey of MTE and how modern software such as {\tt glibc} and {\tt Android} makes use of MTE for memory safety. We identified some common weaknesses in the implementation of memory tagging across various systems and propose improvements. We also proposed simple enhancements to MTE to improve its memory safety guarantees. Lastly, we developed and experimented with an architectural improvement to MTE that can strengthen security while still being memory efficient. 

==> eurosp2023-template/abstract.tex <==
\begin{abstract}
ARM recently introduced a security feature called {\em Memory Tagging Extension} or MTE,
which is designed to defend against common memory safety vulnerabilities,
such as buffer overflow and use after free. 
In this paper, we examine three aspects of MTE.
First, we survey how modern software systems, such as Glibc, Android, Chrome, Linux, and LLVM, use MTE.
We identify some common weaknesses and propose improvements.
Second, we develop and experiment with an architectural improvement to MTE that 
improves its memory efficiency.
Our design enables longer memory tags, which improves the accuracy of MTE.
Finally, we discuss a number of enhancements to MTE to improve its security 
against certain memory safety attacks. 
\end{abstract}

% C and C++ are well known for their performance and flexibility, but perhaps even more for their extreme memory unsafety, which forms the most important class of security vulnerabilities today. While a lot of research has been done on detecting memory safety bugs, 
% % both during testing \& deployment of code,
% % While there may be - 
% the existing solutions still suffer from either limited security guarantees, or too much performance or memory overhead to be useful in production. ARM MTE is a recently developed hardware-based memory tagging approach which detects these bugs with low performance overhead, and achieves low memory overhead at the cost of low entropy (i.e. low security). 
% % at the cost of low memory overhead. 
% In this project, we aim to first, survey how various memory allocators implement memory safety on top of MTE, and second, improve MTE's memory - security trade off, by reducing the memory overhead of this technique. Specifically, we will try to use compression techniques to provide better security guarantees while using same or less memory for memory tagging.
%\end{abstract}


==> eurosp2023-template/evaluation.tex <==

To compare the real-world space usage of our adaptive BTree to a tag array, we collected the complete memory allocation trace of five commonly used programs. 
We ran all programs on a t4g.small AWS VM, which has 2 arm64v8 CPUs and 2 GB RAM. 
We used Valgrind to get the list of all memory allocations and de-allocations during program execution, 
along with the virtual addresses of the allocations.
% trace all the calls to glibc (malloc,free etc) and new, delete made during the program execution. Hence we 

Figure~\ref{fig:workload-alloc-cdf} plots the CDF of allocation sizes for all five workloads. 
Table~\ref{tab:workload-stats} lists details of the five workloads, 
along with the number of allocations, average allocation sizes, and the total number of pages used. 
We also report the average number of runs per page, 
calculated by first measuring the maximum number of runs on each page, during the program execution, and then averaging this over all pages.

We remark that to convert the virtual addresses of allocations to physical page addresses we used 4KB pages.
%, and divided virtual addresses and the corresponding allocations into 4KB pages. 
While Linux exposes virtual to physical page mappings via {\tt /proc/PID/pagemap}, 
it can be unreliable due to lazy mapping, copy-on-writes, and page swapping.
We therefore did not use it. 
% Since there's no reliable way of getting physical page mappings of user space virtual addresses. 
We discuss how page size impacts our results in Section~\ref{sec:btree-discussion}.


% and the average number of runs on each page. We 

% We profiled 5 real-world workloads using valgrind, as listed below. Figure \ref{fig:workload-alloc-cdf} plots 

% \begin{figure*}[t]
% \centering
% \setlength{\tabcolsep}{1pt}
%   \renewcommand{\arraystretch}{0.9}
%   \vspace{0.5em}
%   \resizebox{\textwidth}{!}{
%    \begin{tabular}{cc}
%     % \includegraphics[width=0.2\textwidth]{cs_thesis_latex_template-2020/figures/GM_run1.pdf}
%     % & height=0.13\textwidth
%      \includegraphics[]{figures/apache2_Workload_AllocSzHistogram.pdf}
%      &
%      \includegraphics[]{figures/axel_Workload_AllocSzHistogram.pdf}
    
%     \end{tabular}}
%     \vspace{-1em}
%     \caption{Histogram of allocation sizes for Apache (left) and Axel (right) workloads. The y-axis denotes the number of allocations of a particular size, in log scale.}
%     \vspace{-10pt}
    
% \label{fig:workload-alloc-hist}
% % \vspace{-10pt}
% \end{figure*}

\begin{figure}[t]
\vspace{3pt}
\centering
 \includegraphics[width=0.48\textwidth]{figures/All5Workloads_AllocSzCDF_Final.pdf}
 \vspace{-17pt}
    \caption{CDF of allocation sizes for all five workloads. The x-axis denotes allocation size in log-scale.}
\label{fig:workload-alloc-cdf}
% \vspace{-10pt}
\end{figure}

\begin{table}
\caption{\rm Details and Statistics of 5 real-world workloads collected using valgrind.}
\vspace{-5pt}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llllll}
\hline
\textbf{Name}    & \textbf{Description}                                                                 & \textbf{\#Alloc.} & \textbf{Avg Size} & \textbf{\#Pages} & \begin{tabular}[c]{@{}l@{}}\textbf{Avg \#Runs} \\ \textbf{Per Page}\end{tabular} \\ \hline
apache2 & \begin{tabular}[c]{@{}l@{}}Apache bench \href{https://httpd.apache.org/docs/2.4/programs/ab.html}{ab} \\ 20k req.\end{tabular}             & 771      & 1035                                                      & 207     & 6.46                                                           \\ \hline
axel    & \begin{tabular}[c]{@{}l@{}}Download\\ 6KB file\end{tabular}                 & 231      & 144745.7                                                  & 8918    & 4.87                                                              \\ \hline
ffmpeg  & Resize image                                                                & 4734     & 5597                                                      & 6545    & 2.9                                                            \\ \hline
md5sum  & \begin{tabular}[c]{@{}l@{}}Calculate md5 \\ hash of 0.5GB file\end{tabular} & 231      & 265.3                                                     & 19      & 18.32                                                          \\ \hline
pbzip2  & \begin{tabular}[c]{@{}l@{}}Compress 2.5MB file\\ 1thread\end{tabular}       & 34       & 818859.7                                                  & 6800    & 2.01                                                           \\ \hline
\end{tabular}
}
\vspace{-8pt}
% \vspace{-20pt}
\label{tab:workload-stats}
\end{table}

% Each page has 4.6 allocations on average.
% [TODO: any other per-page stats?]
% Figure \ref{fig:workload-alloc-hist} (left) plots a histogram of the allocation sizes for this workload.

% , with 124 allocations on average. [this avg is misleading since it double-counts on re-allocations]
% Figure \ref{fig:workload-alloc-hist} (right) plots a histogram of the allocation sizes for axel.

For FFmpeg, out of 4734 allocations, Valgrind was unable to track 21 allocations of total size 1848 bytes. We manually insert these missing allocations by simulating the worst possible workload for us: we add another page, with 20 allocations of size 16 bytes and 1 of size 1528 bytes, with 16 bytes of metadata between each allocation. 

% \paragraphi{FFmpeg} We used ffmpeg to resize an image. It makes 4734 allocations, out of which After accounting for these missing allocations, we get average allocation size of 5597 bytes. These allocations span ? pages.
% each with ? allocations on average.

% There are 231 allocations, with average size 265.3 bytes and spanning 19 pages.
% , with 13 allocations per page on average.

 % This program makes 34 allocations, with average size 818859.7 bytes, which span 6800 pages.
% with just 1 allocation per page, on average.

% Workload characteristics:
% \begin{itemize}
%     % \item apache: HTTP server
%     % \item axel: file downloading
%     % \item ffmpeg
%     % \item md5sum: checksum
%     % \item pbzip2: file compression.
%     % \item TODO: Add histograms to show alloc size distribution (2 workloads), mean alloc size, \#pages with just 1 allocation.
%     % \item TODO: also discuss avg allocation size vs avg active allocation size??
%     % \item TODO: some metric to show malloc - free trend [active alloc sz might handle this] / 0-tagged metadata. 
%     % \item TODO: mysqld, 
% \end{itemize}


\paragraphb{Setup} 
Before we describe the results, let us briefly explain our setup.
We simulate the 5 workloads on a 2.11GHz x86 machine, based on Glibc and Linux's current implementations of memory tagging. 
% Specifically, we simulate the workloads by, first, initializing all memory with the tag value of 0, i.e. the BTree for each page 

% simulate the workloads based on current impl glibc, linux
As mentioned in \S\ref{sec:btree-impl}, we start with reserving a buffer to store the tags, of the same size as the 4-bit tag array, i.e. 2GB for 64GB RAM. 
We initialize the BTree for each page, with only 1 run starting at 0 and tagged with 0. This mimics Linux's behavior of resetting all memory tags to 0 at initialization. We simulate the workloads by iterating through every malloc/free call as recorded by Valgrind. 

For every new allocation, we call {\sf IRG} (implemented in software using rand()) to generate a new random tag, and then call our {\sf STG} implementation to update the BTrees in the corresponding pages, to tag all the granules in the allocation with the generated tag value. All the granules between allocations are tagged with zero since Glibc tags its metadata with zero. This means that there is a 0-tagged run preceding every allocation with a non-zero tag.

For every de-allocation (free or delete call), we iterate over all the freed granules and call {\sf STG} to update their tags in the corresponding pages' BTrees to zero. This is in line with Glibc's approach of tagging freed memory with zero. We note that our {\sf STG} function tries to merge adjacent runs with the same tag, so freed allocations' runs might be merged with nearby metadata runs since both are tagged with zero.

If at any point during the simulation, the BTree for a page tries to use more space than 128 bytes (reserved buffer space per page), we stop updating the BTree and use an array instead. Lastly, to ensure correctness, we call {\sf LDG} and check the tags of all granules after every allocation/de-allocation call.

% We base our experiments on glibc and Linux current implementation of memory tagging. Specifically,
% \begin{itemize}
    % \item All memory is initially tagged with 0.
    % \item All metadata is tagged with 0 in glibc, so the tag of all granules between allocations is 0.
    % \item glibc tags freed memory with 0 as well. We do the same.
% \end{itemize}
% \begin{itemize}
    % \item We simulate the workload on an x86 machine, 
    % \item Implement irg, stg, ldg in software.
    % \item for every new allocation: call irg (rand()), iterate over all granules in this allocation and call stg to store the tag in the BTree.
    % \item for every de-allocation: iterate over all granules and call stg with tag value 0. Note that since we simulate glibc, freed memory runs can be merged with metadata runs, improving space usage.
% \end{itemize}

\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{figures/Prop_Pages_Using_Btree_New_5Workloads.pdf}
 \vspace{-17pt}
    \caption{Proportion of pages that use the BTree (and never switch to tag array) for 4-bit, 8-bit, 16-bit, and 32-bit tags, across all five workloads. (Higher is better)}
\label{fig:workloads-pages-using-btree}
\vspace{-10pt}
\end{figure}

\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{figures/Perf_BTree_Relative_4bTagArr_New_5Workloads_SlowdownPerc.pdf}
 \vspace{-17pt}
    \caption{Performance overhead (in \%) of the LDG, STG operations on BTree, relative to tag array, both storing 4-bit tags.
    Smaller is better.
    These numbers are based on the average time for these operations across all pages. Note that this is based on an unoptimized, software implementation, and is not representative of a hardware-based implementation.}
\label{fig:workloads-perf}
\vspace{-10pt}
\end{figure}

\paragraphb{The results} 
We compare our data structure to the existing approach of a 4-bit tag array, with respect to 
(i) supporting larger tags within the same amount of space, and 
(ii) Performance: we report the latency of {\sf STG} and {\sf LDG} in our software implementation, along with tree depth.

% Space Usage - Since our implementation uses the same amount of buffer as the 4-bit tag array, we evaluate our design on the proportion of memory for which we can support larger tags, equivalently, number of pages that don't switch to 4-bit tag array when using 4-bit, 8-bit or 16-bit tags with our design
% supporting larger tags,
% - we report tree depth, along with numbers based on our software implementation. Note that our performance is not representative of a hardware implementation of BTrees.
% space usage and performance when we use 4-bit, 8-bit or 16-bit tags. For our design, we also report the number of pages that switch to (4-bit) tag array and the average tree depth as they're correlated with memory and performance respectively.

% TODO: Explain our impl uses same space as 4-bit tag array. 

% : a. Space usage, b. Number of pages for which we use a BT when using 4, 8 and 16-bit tags
% Metrics: total space usage, \# pages for which our dynamic DS saves space by using BTree, supporting larger tags., Also tree depth \& performance.

\paragraphi{Supporting Larger Tags} 
%Our BTree implementation uses the same amount of space as a 4-bit tag array but can support much larger tags. 
Figure \ref{fig:workloads-pages-using-btree} plots the
fraction of pages that do not switch to the 4-bit tag array
% 4-bit tags, for the baseline and 
in our adaptive design with the BTree storing 4-bit, 8-bit, 16-bit, and 32-bit tags, for all workloads.
% This metric is 1 for the tag array since the tag size is 4 bits for all pages.
We make the following key observations from the results:
\begin{itemize}%[leftmargin=1em]
    \item The per-page BTree fits within 128 bytes for 57.9\% to 99.98\% pages, across all workloads and all tag sizes.
    This means that
    our design is able to support 8-bit, 16-bit, and 32-bit tags for 57.9\% to 99.98\% of all pages while using the same memory overhead of 3.125\%. 
    % i.e. BTree able to compress space usage and fit within 128 bytes (space for 4-bit tag array). i.e. 
    Hence, using our approach, we can get stronger security guarantees by using larger tags for at least 57\% (and up to 99\%) of pages, across a wide variety of real workloads.
    % better memory - security trade-off
    
    \item For the Apache, FFmpeg workloads, on varying the tag size from 4-bit to 32-bit, there is a 6\% decrease in the proportion of pages that do not switch to the tag array. This is because, while the structure of each BTree remains the same, the space used by each node in the tree increases with tag size (as described in \S\ref{sec:btree-analysis}). Hence, more pages switch to the 4-bit tag array as their BTrees do not fit within 128 bytes for larger tags. This is expected as per our analysis in \S\ref{sec:btree-analysis}.
    % BTree space usage increases with tag size [as we saw in \S\ref{sec:btree-analysis}], hence, for larger tags: BTree for lesser \% of pgs.
    \item Across different workloads, we observe that the proportion of pages that do not switch to 4-bit tag array increases as the average number of runs per page increases. 
    For instance, md5sum has the largest average of 18.3 runs per page, as compared to pbzip2 which has the smallest average of 2 runs per page. Hence, the md5sum workload has only about $60\%$ of pages that use the BTree. This corroborates our analysis (\S\ref{sec:btree-analysis}) since, for a larger number of runs per page, more pages would have to switch to the tag array as their BTree would not fit within 128 bytes.   
    % BTree for larger \% of pgs if larger avg alloc size.
\end{itemize}

\paragraphi{Performance} For 4-bit tags, LDG instructions in our software implementation take up to $3\%$ more than a basic tag array on average, 
and STG takes up to $12\%$ more. This is across all workloads. Figure~\ref{fig:workloads-perf} plots the average performance of our 4-bit BTree relative to a 4-bit tag array. Note that these numbers are based on our software implementation and are not representative of an ARM hardware implementation. 
The average depth of the BTree is between $1$ and $1.17$ for all workloads and tag sizes, with the max depth being 3 for 4-bit tags and 2 for 8-bit to 32-bit tags.
% varies between 1-3 across all pages for 4-bit and 8-bit BTrees, and between 1-2 for 16-bit BTrees. This is expected as per our analysis that the maximum depth of BTrees that can fit within 128 bytes is 3 for 4-bit tags and 2 for 8-bit, 16-bit and 32-bit tags.

% S/W numbers, but not representative of real performance in H/W. 

% \begin{itemize}
%     \item Assuming same tag size as tag array i.e. 4bits, a. total space used by Tag array vs our dynamic DS. [bar chart: tag array, 4bit tag, 8bit tag for all workloads] b. \#Pages for which BTree was used.
    
%     As expected (based on our analysis), we get much better space savings in workloads with larger average allocation size.
    
%   c. Stats on depth of trees for Performance analysis 
    
%     \item Varying tag size: a. space savings [x: tag size, mem used: y 2*1plot per workload: apache,?], b. \#pages for which we can support large tags by using BTree.  Actual data for 4bit, 8bit, and theoretical numbers for tags larger than 8bits. (Within the same amt of memory reserved for 4-bit tag array.)
% \end{itemize}

% Undefined in per page BTree- Within the same array size, whats the max tag size that BTree allows us to use? As we increase tag size, more and more pages will switch to tag array.

% larger tag, less space savings & we use large tag for lesser #pages.

% Also depends on caching.

% [Now in discussion]
% \begin{itemize}
%     \item Can now support stgm like instructions for user space.
%     \item Enable BTree based storage if a. workload has big allocations, AND b. if higher security guarantees are needed (since slight performance overhead might be acceptable).
% \end{itemize}

==> eurosp2023-template/improvements-additional.tex <==
\section{Additional improvements to MTE}
\label{sec:additional}

\noindent
Finally, we discuss a few additional enhancements to MTE. 

\subsection{H/W Supported Invalid Tags}  
\label{sec:improve-invalid-tag}

In Section~\ref{sec:mte-impl-scudo} we saw that tagging freed memory with a random tag helps detect Use-after-free's with 93\% probability. 
This can be further improved if the hardware supported an explicit {\em invalid} tag:  a tag that causes every access to the granule to raise an exception.
A freed granule can be tagged with this tag so that the hardware will raise an exception on any attempt to access this granule. 
%When an allocation is made, a random tag (excluding the invalid tag value) is generated and used to tag allocated granules. This can give us 100\% protection against use-after-free, 
Since the invalid tag value cannot be used to tag allocated memory, this will leave 15 possible tags for allocated memory (assuming 4-bit tags are used).
%with just a slight reduction in spatial and use-after-realloc from $15/16$ to $14/15$, since  
We note that granules used to store metadata need to be accessible to the allocator and hence will have to be tagged with a random valid tag value.
The invalid tag is akin to an unreadable guard page, however, assigning the invalid tag to a freed granule allows access control at a much finer granularity.


\subsection{Combining PAC and MTE for Memory Safety} % to reduce tag storage
\label{sec:improve-combine-pac-mte}

Recall that ARM PAC (Pointer Authentication Code) embeds a cryptographic integrity tag (a MAC) into the high-order bits of every pointer and return address. This means that for data pointers, we need to store both the MTE tag and the PAC in the pointer.
% , with security depending on the tag size for both memory safety and pointer integrity
A 64-bit pointer has a limited number of unused bits for these tags: 
only 11 to 31 bits can be used to store both the PAC and MTE tags
(32 to 52 low-order bits hold a virtual address and 
the 55th bit is reserved for selecting the high or low half of the virtual address space).

Concretely, for a machine with 47-bit virtual address space, there are \combinedtagsz unused bits; we could either use all \combinedtagsz bits for MTE tags (using our design) or use all the bits for PAC.
More generally, we can use $x$ bits for MTE and $\combinedtagsz-x$ bits for PAC for some $0 \le x \le \combinedtagsz$. 
This presents a tradeoff between memory safety and pointer integrity for data pointers. 
 
 We propose to improve this significantly by combining MTE and PAC for data pointers. 
 By storing a single \combinedtagsz-bit tag in every data pointer we show 
 that the combination provides memory safety similar to a \combinedtagsz-bit MTE 
 and pointer integrity similar to a \combinedtagsz-bit PAC for most of RAM.

% NEW outline:
% P1 (motivation).
% \begin{itemize}
    % \item Recall that ARM PAC (Pointer Authentication Code) embeds a cryptographic integrity tag (a MAC) 
% into the high-order bits of every pointer and return address. This means that for data pointers, we need to store both the MTE tag and the PAC in the pointer, with security depending on the tag size for both memory safety and pointer integrity. But, there are only a limited number of unused bits in a 64-bit pointer: with 32-bit to 52-bit virtual address spaces, and 1 bit reserved for selecting the high or low half of the virtual address space, there are only 11 - 31 bits available to store these tags.

    % \item security of both MTE, PAC depends on the size of the pointer tag but [need to store both MTE, PAC tags in ptr] limited bits in ptr. 
    % \item 
   
    % \item The current architecture allows using upto 8 bits for MTE for memory safety, and the remaining 3-23 bits for PAC to detect pointer corruption. While our design supports using larger MTE tags with the same memory overhead, we would have to use smaller PAC. 
    % \item
    % Concretely, for a ?-bit VA space, . // the security of both these features is 
    % \item We propose to improve this significantly by combining MTE and PAC for data pointers. This can allow using large/upto 31-bit tags for both the features. // allow using larger tags tags for both 
% \end{itemize}

% P2. Recall PAC*2, We look at combining MTE and PAC. Concretely, we assume a 39-bit VA space, leaving 24 bits for MTE or PAC. We show that the combination provides memory safety similar to a 24-bit MTE as well as pointer integrity similar to a 24-bit PAC.
\ignore{
Recall that ARM PAC (Pointer Authentication Code) embeds a cryptographic integrity tag (a MAC) 
into the high-order bits of every function pointer and return address.
This MAC is computed using a secret key known to the processor and is checked whenever the pointer is de-referenced.
While the tag size for MTE is currently limited to 4 bits, 
PAC can use anywhere from 3 to 31 bits.
Fat pointers may enable even longer tags. 
}

% due to TBI only allowing the top byte to be non-zero.
% and PAC using 4 of the 8 available bits. 

% In this section, we look at combining MTE and PAC for data pointers to enhance memory safety. % within the same memory overhead.
% To be concrete, we assume that 16-bit PAC is used, as is the default in AArch64 Linux.
% We show that the combination provides security similar to a 16-bit MTE tag,
% but at the cost of storing only a 4-bit MTE tag in memory.
% //

\ignore{
\paragraphb{Design} Consider the following way of combining the bits for PAC and MTE into a single \combinedtagsz-bit pointer tag for data pointers. Let $t_p$ and $t_m$ denote the \combinedtagsz-bit pointer tag and \combinedtagsz-bit MTE memory tag respectively. 
}

\ignore{
\paragraphb{Design}
Consider the following way of combining the bits for PAC and MTE into a single 16-bit pointer tag for data pointers.
%(which is possible if the Top Byte Ignore feature is extended to 2 or more bytes). 
Let $t_p$ and $t_m$ denote the 16-bit PAC pointer tag and 4-bit MTE memory tag respectively. 
}

\paragraphb{Design} 
Let $k$ be a PAC secret key known to the processor.
Whenever a new allocation is made at address $a$,
the memory allocator generates a fresh random \combinedtagsz-bit MTE tag $t_m$. 
Next, the processor generates a \combinedtagsz-bit PAC tag $t_p$ as follows:
\[
    t_p \gets \text{QARMA}\bigl( k, (t_m, a) \bigr).
\]
Here QARMA is the block cipher used in PAC (128-bit key and 64-bit block size),
where the output of QARMA is truncated to \combinedtagsz bits.
This $t_p$ is embedded in the high-order bits of the returned pointer.
The system can include additional context (such as the object type~\cite{ccfi,pac-parts-sec19,pac-security22}) 
as further input to the cipher.
%When memory is freed, the processor generates a new random \combinedtagsz-bit memory tag but the freed pointer remains unchanged.

%Note that the pointer tag $t_p$ can be larger than the memory tag $t_m$. 
In addition, for every allocation, the processor stores the allocation's starting address $a$ and the \combinedtagsz-bit memory tag $t_m$
in the adaptive data structure from Section~\ref{sec:btree-design}.
Hence, this scheme has exactly the same memory overhead as if MTE used 4-bit tags. 
Looking up any address in the data structure returns the starting point $a$ of the enclosing allocation along with $t_m$. 
For pages where 
% the BTree does not fit within the reserved buffer space, 
the system switches to a tag array, the processor stores the lower four bits of $t_p$, which we denote by $t_m'$. 
This is closely related to PACSan's~\cite{pacsan-arxiv} pointer tags, 
but our data structure for storing metadata in memory is different and provides better support for caching, pre-fetching, and page swapping.

At every load/store instruction, the system compares the \combinedtagsz-bit pointer tag $t_p$ to $\text{QARMA}\bigl(k, (t_m, a)\bigr)$ 
where $(t_m, a)$ are obtained from the page's BTree.
Here $a$ is the starting address of the allocation containing the address in the pointer,
and $t_m$ is the MTE tag of that allocation.
If the page has been switched to a tag array, the system compares the lower four bits of $t_p$ to the 4-bit $t_m'$ stored in the tag array. 
In this case, the scheme reduces to regular MTE.

\ignore{
Note that we are comparing 16-bit tags, even though only a 4-bit $t_m$ is stored in memory 
(the address $a$ is always stored in the BTree irrespective of the tag length). 
}

% At alloc: r, a0 -> t in ptr.
% This tag is generated using 
% QARMA, start address as modifier/context, use the same data structure as described in \S\ref{sec:btree-design}. As shown in \S\ref{sec:btree-storage-eval}, limited mem overhead.

% Label should always be after caption!!! Otherwise, table # is wrong.
\begin{table}
\begin{center}
\vspace{7pt}
\caption{\rm Security Analysis of MTE vs. PAC+MTE vs. PAC all using \combinedtagsz-bit tags. We list the memory overhead for storing a single run in the BTree. For every attack, we list the probability (in \%) of a benign or malicious attempt being detected. We assume random re-tagging on free. PAC+MTE provides the benefits of a 16-bit PAC and a 16-bit MTE, while only using 16 bits.}
\vspace{-5pt}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{llll}
% \hline
         & \begin{tabular}[c]{@{}l@{}}\textbf{MTE \combinedtagsz-bit}\\ $|t_m| = \combinedtagsz$\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{PAC+MTE}\\ $|t_p| = \combinedtagsz = |t_m|$\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{PAC \combinedtagsz-bit}\\ $|t_p| = \combinedtagsz$\end{tabular} \\ \hline
Memory Overhead     & (\combinedtagsz,$|a|$)  & (\combinedtagsz,$|a|$)     & 0   \\ \hline
Linear Overflow     & 99.9   & 99.9  & 0    \\ \hline
Non-Linear Overflow & 99.9   & 99.9   & 0    \\ \hline
Use-after-free      & 99.9   & 99.9    & 0     \\ \hline
Use-after-realloc   & 99.9   & 99.9    & 0     \\ \hline
Pointer Corruption  & 0    & 99.9  & 99.9  
\end{tabular}
}
\end{center}
% \vspace{10pt}
\label{tab:combine-pac-mte-security}
% \vspace{-15pt}
\end{table}

\paragraphb{Security}
Table \ref{tab:combine-pac-mte-security} compares the protection provided by MTE, PAC, and PAC+MTE
against memory unsafety and pointer corruption.
In all three examples we use \combinedtagsz-bit pointer tags.
% As per \S\ref{sec:btree-storage-eval}, the number of pages that don't switch to tag array for the MTE with 8-bit tags, would be smaller than MTE as well as PAC+MTE with 4-bit memory tags.
% We use 4-bit memory tags for both schemes to keep their memory overhead equal, for a fair comparison.

For overflows into adjacent or non-adjacent allocations, 
MTE can detect both benign and malicious attempts with a probability of at most $65535/65536$.
% $15/16$ (93\%) when a 4-bit $t_m$ is used, and $65535/65536$ when a 16-bit $t_m$ is used.
For PAC+MTE, the probability of the overflow succeeding is $1/65536$.
This is because the attacker can, at best, guess the \combinedtagsz-bit MAC $t_p$ with probability $1/65536$, 
even if they know the starting address ($a$) of an allocation.
Hence, PAC+MTE is able to provide the same spatial safety as MTE.
% with 16-bit tags, 
% by only storing a 4-bit MTE tag $t_m$.

For Use-after-free, if freed memory is tagged with a random tag $t_m$, 
MTE provides $65535/65536$ protection.
% , for 4-bit and 16-bit tags respectively.
For PAC+MTE, if a dangling pointer (with tag $t_p$) is used to access freed memory, 
the BTree will return the same starting address (since freed memory also forms a run with the same address but just a different tag), 
but the memory tag will be different. 
As a result, a benign or malicious UAF attempt will succeed with $1/65536$ probability. The analysis is similar for Use-after-realloc. PAC+MTE therefore provides the same temporal safety as MTE.
% In other words, PAC+MTE does not buy us much in defending use-after-free.

%The analysis for Use-after-realloc is similar for all schemes.

% \begin{equation}
%     t_p = \text{QARMA}(k, t_m', a_l)
% \end{equation}

% Lastly, for Use-after-realloc, both MTE and PAC+MTE schemes can detect benign and malicious with 93\% chance, since if the starting address of the allocation remains the same, there are only 16 different possible values of $t_p$, based on 16 values of $t_m$. So, there is a 1 in 16 chance of the tags matching after re-allocation.

In terms of pointer corruption, an attacker can only guess the correct PAC for a new address with probability $1/65536$. Hence, PAC+MTE provides the same pointer integrity as PAC with \combinedtagsz-bit pointer tags.

In summary, the PAC+MTE scheme uses larger pointer tags, which, combined with the data structure from Section~\ref{sec:btree-design}, 
can provide stronger memory safety and pointer integrity for 57\% to 99\% RAM, with the same memory overhead as MTE with 4-bit tags. Note that pointer reuse attacks are possible in both PAC and PAC+MTE schemes, but they can be made harder by including additional context in the MAC,
such as the allocation size and object type.
% more spatial, equal temporal for all pgs that dont switch, with same memory tag size.
\ignore{
Note that for a given address~$a$, the \combinedtagsz-bit $t_p$ is always one of 65536 possible values determined by the \combinedtagsz-bit $t_m$.
If the attacker could obtain all 655 possible values for $t_p$ at $a$, 
then all protection probabilities revert to $15/16$. 
}


==> eurosp2023-template/improvements-new.tex <==
%\vspace{-10pt}
\section{Improving MTE's memory efficiency}
\label{sec:improvements}  
% \subsection{A proposal for additional features}

%% Hardware support for invalid tag, to prevent use-after-free.
%% Stack tagging.
%% k-wise independence for tag generation
% Define 0 as an invalid tag. This tag value is already reserved since its overhead is higher than other tag values. 
% \begin{itemize}
    % \item Dont use it for any newly allocated memory
    % \item Assign this to freed memory - trying to access memory tagged with invalid tag causes exception. i.e. if ptr tag = invalid\_tag, throw exception. Deterministic 
    % \item But if freed chunks storing metadata: use some other tag value
    % \item This is similar to how scudo's secondary allocator tags freed memory with PROT\_NONE, but invalid tag can let us do the same thing at a much finer granularity.
% \end{itemize}
% We can extend Linux SLUB's invalid tag idea to hardware. If we could allow the user to define a particular tag as invalid (similar to how MTE allows using a match-all tag), it can provide a stronger security guarantee against use after free attacks, by assigning this invalid tag to freed memory. 
% For malloc: dont use tag 0 for tagging new allocations, at realloc: mem tag updated to new value.
% Provides deterministic protection against UAF attacks.

% \subsubsection{Pair-wise Independent Tags}
% [TODO] Use fixed random bits for a page/process? to generate tags of allocations.
% Would need to store alloc\# in a BTree? to generate tag of an addr at ldg/stg.

\label{sec:improve-btree}

Since MTE uses 4-bit tags, there is a 1 in 16 chance that a random rogue pointer will contain the correct tag. 
While there is room in the high-order bits of a 64-bit pointer to store longer tags~\cite{linux-tag-addr-abi,arm-pac-whitepaper},
the reason MTE uses such short tags is due to the overhead of storing all tags in memory.
With a 4-bit tag for every 16-byte granule, this overhead is already 3.25\%. 
Concretely, the tag array takes 2GB for a machine with 64GB RAM. 

We propose to improve this significantly by compressing the tag storage using a succinct data structure instead of a tag array.
This lets us use longer tags without taking up additional storage in RAM. 

% We begin with detailing our data structure design in \S\ref{sec:btree-design}, followed by implementation \S\ref{}, analysis, evaluation, discussion.

% \begin{itemize}
%     \item MTE's security is limited since it uses only 4 bit tags to limit the memory overhead. Probabilistic attacks succeed with 7\% probability.
%     \item We can improve this security - memory tradeoff by compressing the tag storage
% \end{itemize}

\begin{figure}[t]
\centering
 \includegraphics[width=0.48\textwidth]{figures/All5Workloads_Avg_v2_NoErrBar.pdf}
 \vspace{-10pt}
    \caption{Average allocation size of real-world workloads. The y-axis is in bytes, in log scale.}
\label{fig:workloads-avg}
\vspace{-10pt}
\end{figure}

\subsection{Our approach}
\label{sec:btree-design}

For a large allocation, say 160 bytes, it can be wasteful to store the same tag value in the tag array for all 10 granules in this allocation. 
Figure~\ref{fig:workloads-avg} shows the average allocation sizes for five real-world workloads running on an Arm64v8 VM. 
We observe that the average size lies between 265 and 818859 bytes (17 to 51179 granules).
This means that a lot of space is wasted by storing the same tag 17 to 51179 times on average.
We could instead use Run Length Encoding (RLE) to store the starting address and tag value for each run, 
as shown in Figure \ref{fig:rle-example}. 
Each continuous set of granules with the same tag is called a run: the example in Figure~\ref{fig:rle-example} has 6 runs.
% Using RLE to store tags is analogous to storing per-object metadata as done in~\cite{aos-micro-20,pacsan-arxiv}.

Storing the RLE encoding instead of an explicit tag array greatly reduces the memory space needed to store tags. 
Consequently, we could either store 4-bit tags in less memory, or use larger tags, say 8, 16, or even 32 bits per granule, 
without expanding the total memory used by MTE. % compared to the current tag array implementation. 
However, an RLE-based data structure is useful only if 
(i) reading the tag of a granule is fast (needed in every load and store instruction), and
(ii) maintaining the data structure as tags are updated is efficient (needed in every memory allocation/de-allocation).

Our approach supports both properties, while maintaining low memory overhead. 
We do so by using a suitable BTree to store the starting addresses of all runs, along with their corresponding tag values. 
The starting addresses are used as the keys for the tree. 
Figure \ref{fig:rle-btree-example} shows a 4,5-BTree for the tag array in Figure~\ref{fig:rle-example}. 
With this data structure, accessing and modifying the tag of a random granule takes time proportional to the depth of the BTree.
%which depends on the number of keys in the tree. 
As the number of runs stored in the tree increases, so does the depth of the tree.
As we will see in \S\ref{sec:btree-storage-eval}, the depth of the BTree stays quite small in most real-world workloads. 
Hence, we are able to support larger tags without exceeding the memory overhead of a 4-bit tag array, 
while supporting fast tag access and update. 

With this approach, every pointer will need to store a larger tag in its high-order bits.
We explain how to do that in Section~\ref{sec:btree-discussion}.

In Section~\ref{sec:usage-survey} we saw that allocators try to improve the running time of malloc and free by
minimizing the number of times that they update the tags associated with the granules of a large buffer.  
The BTree data structure has the added benefit that a single update to the tree
can update the tags of many consecutive granules.
This may make it unnecessary to employ the security-harming optimizations used by some allocators.


\paragraphb{Using a per-page BTree}
There are three difficulties with using a global BTree for the whole of RAM. 
\begin{itemize}%[leftmargin=1em]
\item Concurrency:
If two processes own adjacent physical memory pages, then it becomes difficult to concurrently update tags for their granules.
This is because the runs for these processes might belong to the same sub-tree or the same node, and hence we might need to use extensive locking. 
While lock-free implementations of BTrees exist~\cite{bw-tree-msr}, they are inefficient and complex to implement~\cite{bw-tree-hard-sigmod}. 

\item Page swaps: 
Whenever the OS swaps a page between memory and disk, the tags corresponding to that page also need to be swapped. 
With a global BTree, this will require reading the tag of every granule in the page, writing it to disk, 
and then updating the global BTree with the tags of all the granules read from disk. 
This can be an expensive operation and combined with the first issue, can affect adjacent pages as well. 

\item An attack:
A global BTree is susceptible to an algorithmic complexity attack~\cite{algo-comp-attacks}, 
where a single process can make a large number of small allocations to increase the size and depth of the tree, 
thereby slowing down all the other processes on the machine. 
For example, if process~1 and process~2 both have one page each, and process~1 only has one allocation, 
then the depth of the BTree would be 1 if process~2 only made one allocation.
However, the depth of the global tree increases to five if process~2 were to make 256 16-byte allocations on its page.
\end{itemize}

\medskip\noindent
To address the difficulties with a global BTree, we opt for a separate BTree for every page. 
This allows different processes to concurrently access and modify the BTrees corresponding to their pages (except for when pages are shared among processes).
Page swapping can be easily done by copying the corresponding BTrees in or out of memory. 
Lastly, a process with a large number of allocations per page will only slow down other processes sharing the same page. 
The only downside is that a per-page data structure takes up a bit more memory than a global BTree, because allocations larger than a page are now split into multiple runs, i.e. one run in the BTree of each page.
But, our experiments show that we can still support large tags without expanding the memory used by MTE. 

\begin{figure}[t]
\centering
 \includegraphics[width=0.47\textwidth]{figures/BTree_example_RLE.pdf}
%  \vspace{-10pt}
    \caption{Run Length Encoding Example. We have 3 allocations, each of size 48 bytes (three granules), with one granule of Glibc metadata before every allocation.}
\label{fig:rle-example}
% \vspace{-10pt}
\end{figure}

\begin{figure}[t]
\centering
 \includegraphics[width=0.25\textwidth]{figures/BTree_example_BTree.pdf}
%  \vspace{-10pt}
    \caption{BTree corresponding to the tag array in Figure \ref{fig:rle-example}}
\label{fig:rle-btree-example}
% \vspace{-10pt}
\end{figure}

\paragraphb{An adaptive data structure} 
The BTree structure can greatly reduce the space requirements when there are few allocations on a page, 
namely when the average allocation size is large. 
However, the BTree may grow too large if a process makes a large number of small allocations. 
If left unchecked, this can increase the memory overhead and slow down accesses and updates to memory tags for that page,
as explained in Section~\ref{sec:btree-analysis}.

To prevent this from happening, we take an adaptive approach.
If the memory usage of the BTree for a page crosses a certain threshold, 
the system switches that page to an explicit tag array that stores 4-bit tags, as in the current MTE implementation. 
This bounds the memory overhead of our design.


% \begin{itemize}
%     % \item intuition: for allocation of consecutive buffer in a physical page  - no need to store the same tag for all granules separately. -> RLE.  
    
%     % \item This greatly reduces the memory space needed to store tags.  Consequently, we can use larger tags, say 8 or even 16 bits per granule, but still use the same amount of memory as the current tag array implementation. 
    
%     % \item The challenge: how to maintain RLE when tags are constantly changing??
%     % \item The solution: build a btree to succinctly store all the runs.
%     % \item Dynamic: for any page, switching to array if the btree size crosses a threshold.
%     \begin{itemize}
%         % \item Only store the last 4 bits in tag array.
%         % \item Pointers would still need to store the large tag, and MMU can decide how many bits to use.
%         \item Cannot move back to the BTree since the upper bits are lost. Once the page is re-allocated (e.g. when kernel resets tags to 0 by calling STGM), we can move to a BTree. TODO: We could potentially add a new instruction to tell the H/W to reset the tags and switch to a BTree.
%         % \footnote{We could potentially ad a }
%     \end{itemize}

%     % \item Per page vs Global BTree 
%     % \begin{itemize}

%     %     \item Multi processing : would require locking in global BTree. While lock-free implementations of BTrees exist, such as BW-Tree, they are known to be very hard to implement.
%     %     \item Handling page swapping : Global BTree: will have to read the tag of every granule in the page, write to disk, zero them out, then write the tag all granules read from disk to the global BTree. It would be much easier to just copy the whole data structure for the page being swapped in/out.
%     %     \item Algorithmic Complexity Attacks: An attacking process could make a lot of small allocations. Todo: add example with theoretical numbers. Attack still possible for shared memory but limited to 1 page only With a per page BTree, an attacker can only affect processes sharing the same page.
%     % \end{itemize}


% \end{itemize}

\subsection{Implementation}
\label{sec:btree-impl}

We now describe the implementation of our per-page adaptive BTree data structure. 
We aim to support larger tags with the same memory overhead as an explicit 4-bit tag array. 
Our implementation supports 4-bit, 8-bit, 16-bit, and 32-bit tags.
The desired tag size can be chosen at boot time.

An alternative design could instead continue to use 4-bit tags, as currently used by MTE,
and focus on reducing the overall memory requirements.
We do not do that since this would make it much harder to locate the metadata for each page in memory.
Instead, we place the metadata for each page in a fixed location in RAM and aim to use larger tags. 

\medskip
Recall that the default page size for Linux on AArch64 is 4KB.
We assume all pages are of this size, and discuss the impact of variable page sizes in Section~\ref{sec:btree-discussion}.

\smallskip
\paragraphb{Tag Storage}
We reserve a buffer of the same size as the 4-bit tag array for the whole RAM, i.e. 2GB for a machine with 64GB RAM. We fit our BTree data structure with large tags, within this buffer. The BTree for each 4KB page gets 128 bytes (equal to the tag array space for the page), and the tree for the $i$th page is contained between [128i, 128(i+1)] bytes of the buffer.

 \begin{lstlisting}[language=c, caption={The struct defining a node in our per-page BTree for 4KB pages.}, label={lst:btree-node}]
  struct BTreeNode {
    unsigned char keys[4];
    unsigned char children[5];
    unsigned char parent;
    unsigned char tags[TAGARR_NUM_BYTES];
    char count;
  };
\end{lstlisting}

\paragraphb{BTree Implementation}
We build a 4,5-BTree for each page, consisting of nodes as defined by the struct in Listing~\ref{lst:btree-node}. Each node contains the following fields: 
(i) an array of size 4 for storing upto 4 keys. 
Since each key is the start address (granule number) of a run, and there are 256 granules in a 4KB page, 
the key is in the range 0 to 255, and can fit in an 8-bit char. 
(ii) an array of child pointers, of size five, since each node can have up to five children. Each child pointer points to another node in the BTree, and we store the pointer as a relative offset from the starting address of the buffer for the BTree (which is $128i$ for the $i$th page). 
So, the child pointer is in the range 0 to 127, and we store it in an 8-bit char.
(iii) a parent pointer, which also stores the relative offset instead of the absolute address, and hence fits in an 8-bit char. 
(iv) the tags corresponding to each key. The value {\tt TAGARR\_NUM\_BYTES} depends on the tag size: 
we need 2 bytes to store four 4-bit tags, and 4, 8, and 16 bytes to store four 8-bit, 16-bit, and 32-bit tags respectively. 
Lastly, (v) we store the number of keys in the node in a separate field called count. 

% Listing \ref{lst:btree-node} lists the struct defining all the fields in a BTree node. 
Each node in the per-page BTree takes a total of 13, 15, 19, and 27 bytes if 4-bit, 8-bit, 16-bit, and 32-bit tags are used respectively. 
This means that our per-page BTree can only have between 4 and 9 nodes for it to fit within the 128 bytes of reserved metadata space for the page.

For each BTree, we also store additional metadata to manage the space used by the nodes within the buffer (detailed in Appendix~\ref{sec:app-impl}).

\ignore{  %%%  this is a little too much information
\paragraphi{Other Metadata}
For each BTree, we also store additional metadata: the root pointer, as a 1-byte value, denoting the relative offset of the root node from the start of the buffer for this BTree. To manage the allocation and de-allocation of nodes as the tree grows, we use a 2-byte bit array to denote which nodes in the 128-byte buffer are free. 16 bits are enough since only 4-9 nodes can fit within the 128 bytes buffer. Lastly, we have an additional 1-bit flag for each page, denoting whether we are using a BTree or an array for storing tags for that page.

\paragraphb{Initialization}
We initialize the BTree data structure with the root at offset 0, and all the bits in the free nodes bit-array (except 0th) are marked free. 
The root only has one key: 0, with tag value 0, meaning that the whole page is tagged with 0.
}

\paragraphb{Handling Tag Accesses}
We implement the {\sf STG} and {\sf LDG} functions, i.e. setting and getting the tag of a single granule, by using BTree algorithms for inserting/deleting keys while keeping the tree balanced. The {\sf STG} function additionally tries to merge adjacent runs with the same tag, to reduce the memory overhead.
% Algorithm~\ref{alg:btree-stg} lists the pseudo-code for the STG function.
% It checks runs neighboring to the granule and merges runs if the tags match.
% It internally uses .
The {\sf LDG} function simply finds the largest key left to the granule (this is the starting address of the run that the granule belongs to), and returns its tag. 

\paragraphb{Switching to a 4-bit Tag Array}
The system monitors the total space used by the BTree and switches to the 4-bit tag array if the space usage exceeds the max buffer size of 128 bytes. 
If that happens, the system switches a 1-bit flag denoting that the page's tags are now stored in a tag array. 
It iterates through all the allocations stored in the BTree and stores the lower 4 bits of each tag in the explicit tag array. 
Hence, the total space used for storing all the tags for the page never exceeds 128 bytes, as in the current MTE.
%We haven't implemented the inline conversion of a BTree to an array, and leave that to future work.
% We can iterate through all the allocations in the BTree and copy only the last 4 bits of the tag into the tag array. 
% We keep a 1-bit flag for each page denoting whether we use a BTree or an array for the page.

We stress that every pointer continues to store the full (4, 8, 16, or 32-bit) tag in its high-order bits. 
The MMU decides how many high-order bits to use based on the
current state of the page being accessed: a BTree or a tag array.
If the page uses a 4-bit tag array, then only the lower four bits of the pointer tag will be used when checking the tag.
We note that it is possible that two objects which had different tags might end up having the same tag after the switch if the lower 4 bits of their tags were equal. This still provides security equivalent to using 4-bit tags.

Once the system shifts a page from a BTree to a \mbox{4-bit} tag array, 
it cannot switch back to the BTree that holds larger tags.
This is because the data required to move back is no longer available in memory. 
The system will reset the page back to a BTree only once the page is released to the operating system. 
% - this could be done by the kernel when it resets the tags on assigning the page to a new process.
% TODO: how?



% We first find the largest key less than the granule's location (i.e. allocation just left to this granule) and similarly the allocation just right to it.  
% If the tag of the granule matches the tag of its left or right key and the key , we merge the two runs.

% \begin{itemize}
    % \item Global buffer of size RAM/32 reserved (same as tag array), page i's buffer space starts at i*128 offset.
    % \item For each page: 1 bit denoting whether we're using BTree or Tag array. This can be a per page flag, similar to 
    % \item BTree Node containing 8-bit keys, children, parent pointers and 8-bit count value.
    % \item Store 8-bit root offset within the page buffer, 
    % 16-bit bool array denoting which nodes are free.
    % \item Tags: Support 4bit and 8bit tags (by disabling PAC) for now. Stored in the node, one tag per key. So, the size of a single BTree node for a 4KB page with 4-bit tags would be 13 bytes.
    % \item Initialize: root at 0, containing  
    % \item Modify stg, ldg instructions to call corresponding BTree functions.
    % \item Maintain first\_avail value, to track how much total memory has been used so far.Note that since during execution, some BTree nodes might be freed: we maintain a 2byte bit-array to store which node offsets are free. This avoids fragmentation in BTree's memory usage. We also store the number of freed nodes as a 1 byte value, to simplify the implementation. We note that this and the first\_avail can be removed at the cost of slightly worse performance. Update jul31: only store bitarray to track freed nodes.
    % \item Switch to tag array if BTree tries to use more than the buffer space for the page (128bytes for 4KB page)
% \end{itemize}

\subsection{Space usage analysis}
\label{sec:btree-analysis}
Next, we analyze the space usage and performance of the adaptive BTree design.
We focus on 4KB pages.

Let $g$ denote the total number of granules on the page. Since each page is 4KB, we get $g = 256$. Let $n$ be the number of runs on the page, wherein each run refers to a contiguous set of granules all tagged with the same tag value. For example, each allocation tagged randomly will form a run, and for Glibc, each metadata granule with tag 0 will form a separate run between allocations. Let $t$ denote the tag length (in bytes) for tags being stored in the BTree. This can be 0.5, 1, 2, or 4 bytes. Let $d$ denote the depth of the BTree storing the starting addresses and tags for all $n$ runs. Let $m$ be the number of nodes and $S^{BTree}_t$ be the total space used to store the tree for $t$-byte tags. 
% Lastly, let $S_t^{Arr}$ denote the space used by the tag array to store $t$-byte tags for each granule, i.e. $S_t^{Arr} = gt$ bytes.
% \paragraphb{Analysis for 4KB Pages}
% For 4KB pages with 4-bit tags, $S_t^{Arr} = 256*0.5 = 128$ bytes.

\paragraphb{Space Usage} 
% [TODO: keep 1 formula.]
The total space used by each BTree node is $11 + 4t$ bytes, e.g. 13 bytes for 4-bit tags.
Accounting for all $m$ nodes, the metadata, and the fact that each node has at least 2 runs and at most 4 runs, we get the following inequality for the total space used by the BTree (more details in Appendix~\ref{sec:app-analysis}) :
\begin{equation}
\label{eq:btree-space-bounds} 
  \frac{n}{4}(11 + 4t) + 3.125 \leq S^{BTree}_t \leq \frac{n+1}{2}(11 + 4t) + 3.125
\end{equation}
For example, for a 4KB page with 4-bit tags ($t = 0.5$), we consider two cases:
one with $n=2$ runs on the page, and one with $n=256$ runs on the page. 
\begin{itemize}%[leftmargin=1em]
\item 
For $n=2$ runs: the tree has just one node, and the total BTree space is 16.125 bytes.
This is $7.9\times$ smaller than the 4-bit tag array space for the page (128 bytes). 

\item
For $n=256$ runs (the worst case number of runs): using Eq.~\eqref{eq:btree-space-bounds} we have $S_t^{BTree} \geq 835$ bytes, 
meaning that the tree will not fit within the allotted 128 bytes.
\end{itemize}

\paragraphb{Switching to Tag Array} 
For each page, the system switches from a BTree to a tag array if the space usage of the BTree exceeds 128 bytes. 
Considering that each node takes $11 + 4t$ bytes, only $m \leq 9, 8, 6$ and $4$ nodes can fit within 128 bytes, 
for 4-bit, 8-bit, 16-bit, and, 32-bit tags respectively. 
Since each node can only store a maximum of 4 runs, the maximum number of runs that can fit within 128 bytes is 
\begin{equation} \label{eq:th}
  n \leq 36, \quad  n \leq 32, \quad n \leq 24, \quad n \leq 16, 
\end{equation}
for 4-bit, 8-bit, 16-bit, and, 32-bit tags respectively. 
% This gives us $m \leq 9.6$, $m \leq 8.32$ and $m \leq 6.6$ for 4-bit, 8-bit and 16-bit tags respectively. After rounding these values and using Eq \ref{eq:btree-node-run-eqn}, we get that the maximum number of runs that can fit within 128 bytes is 
The system will switch the page to a tag array if the number of runs $n$ on the page exceeds these thresholds at any point during program execution.
% our design will switch it to tag array.
% Note that since the page size is fixed to 4KB, more runs means smaller run size on average, meaning that

The switch thresholds in \eqref{eq:th} decrease as tag size increases.
Hence, one might expect that larger tags will cause more pages to switch to a tag array. 
We test this out by experiment. 


%We note that it is possible for a page to switch to a tag array before $n$ reaches these thresholds, based on the BTree structure and number of nodes used to store those many runs. 
% , since a given number of runs can be arranged in many different BTree structures.

% get bounds on n/m for each t.

% Comparing this to the space used by the tag array, the relative space saving is given by 

% \begin{equation}
% \label{eq:btree-rel-space-savings}
%     \frac{ 2.75n + nt + 3.125 }{gt} \leq \frac{S_t^{BTree}}{S_t^{Arr}} \leq \frac{5.5n + 2(n+1)t + 8.625}{gt}
% \end{equation}

% Let us denote by $g/n$ the average run size on the page, in terms of number of granules. 

% We can make the following two observations from Eq~\ref{eq:btree-rel-space-savings}, that the relative space savings : a. improves as the tag size $t$ increases, for fixed $n,g$. b. improves as $n$ decreases, for fixed $t,g$, i.e. we save more space if the average run size $g/n$ (in terms of number of granules) is larger. Hence, it is better to use a tag array if there are a large number of runs on the page, specifically, the BTree storing 4-bit tags can fit within 128 bytes only if the number of runs is less than 30.

%  Mention when is it better to use Tag array.
 
% Relative Space savings are a. better with larger tags, b. better with larger avg allocations,

% Example : 8 big alloc vs 256 small alloc.

\paragraphb{Performance} 
The running time of the {\sf STG} and {\sf LDG} instructions depends on the depth of the tree. 
Given the size constraints, the BTree depth is at most $3$ for 4-bit tags,
and at most $2$ for larger tags.  
Hence, tree reads and updates are quite fast.
Note that we are unable to experiment with a true ARM hardware implementation of the system.
%we cannot measure the true running time of this design 
%However, we expect it to perform well.

%The performance of this data structure, specifically the {\sf STG} and {\sf LDG} functions, depends on the depth of the tree. Using the fact that each node must have atleast 3 child nodes, we get that $3^{d-1} \leq m$. Combining this with the bounds on $m$, we get that $d \leq 3$ for 4-bit tags, and $d \leq 2$ for 8-bit, 16-bit and 32-bit tags. Hence, all BTree operations will take upto $\theta(3)$ time. This means that the time complexity of accessing and modifying our data structure will be constant time both before and after switching to tag array.

\ignore{
We first analyse the number of nodes $m$ as a function of the tree depth $d$.
The following equation lists the minimum and maximum number of nodes that a tree of depth $d$ can have :

\begin{equation}
    3^{d-1} \leq m \leq \frac{5^d - 1}{4}
\end{equation}

This gives us that $log_5(4m+1) \leq d \leq 1 + log_3m$. 
}
% Since $m \in [\frac{n}{4}, \frac{n+1}{2}]$, we get that $d$ is $\theta(log n)$. 
% Hence, all BTree operations are logarithmic in the number of runs -  a smaller $n$ (or larger average run size) improves performance as well as space savings.
% Max tree depth:
\ignore{
Specifically, for 4-bit tags, we saw earlier that $m \leq 9$, this implies $d \leq 3$. Similarly, for 8-bit tags, $m \leq 8$ gives us $d \leq 2.89$, and for 16-bit tags, $m \leq 6$ gives us $d \leq 2.63$. To summarize, the maximum depth of the BTree that can fit in 128 bytes is 3 for 4-bit BTrees and 2 for 8-bit and 16-bit BTrees.}

% \paragraphb{Generalizing for different page sizes} [TODO] We first generalize the size of a single BTree node for arbitrary page sizes. For a page of size M bytes (i.e. $M/16$ granules), the keys can be stored in $log_2(M/16)$ bits, since they will be in the range $[0, M/16 - 1]$. Similarly, since the child and parent pointers' offsets are limited by the size of the 4-bit tag array for the page, they can be in the range $[0, M/32 - 1]$, and hence can be stored in $log_2 (M/32)$ bits. The total space used by a BTree node will be $4log_2(M/16) + 5log_2(M/32) + log_2(M/32) + 1*8 + 4t*8$ bits. The root offset can also fit in $log_2(M/32)$ bits, similar to the child and parent pointers' offsets. Lastly, the freed nodes bit array would be TODO! [complex formula!]
% We update Eq~\ref{eq:btree-space-usage-1} to 
% \begin{equation}
% \label{eq:btree-space-usage-pg-sz}
%     S^{BTree}_t = m*(10log_2M + 4t - 45) + ? + ? + 0.125 \text{ bytes}
% \end{equation}
% \begin{itemize}
    % \item Let n = number of allocations/runs, g = number of total granules in a page, m = number of nodes in the BTree. TODO: use d for depth!!! m = no. of nodes in tree.
%   \item $#runs=n, #nodes=m, depth=d$.

    % \item Space Usage: BTree: 15*8*m bits. Relative Savings vs Tag array.
    % \item 
    % \item Theoretical example(s) for large allocations on a page. 8 alloc vs 256 alloc.
    % \item Add page size as well?
    % \item Performance: \~ O(log d) : formula for d.
% \end{itemize}

\subsection{Evaluation and Experiments}
\label{sec:btree-storage-eval}
\input{evaluation}

\subsection{Discussion}
\label{sec:btree-discussion}
\paragraphb{Effect of Page Size} For our evaluation, we assumed that all pages are small, i.e. of size 4KB, but Linux supports using huge pages of sizes 64KB -- 1GB on arm64. 
With larger page sizes, we would expect similar or better results because (i) large allocations will be split up into lesser pages, leading to lesser runs per page on average, (ii)
% metadata regarding root offset will be lesser, c. 
% while the size of each BTree node will increase proportional to log of the page size,
as the buffer space for each page will increase proportional to the page size, we will be able to fit the BTrees for pages with larger number of runs as well, e.g. for pages of size 64KB for 4-bit tags, each node will be of size 23 bytes (with 16-bit keys, and child, parent pointers), and the buffer space will be 2KB, meaning that BTrees with over 80 nodes can fit within this space before overflowing. Hence, we will be able to support BTrees with large tags for even more pages than our results for the 4KB page size.
% 2byte root offset, first avail, 23byte node - can fit >1000 nodes in the tag array buffer for the page.

% , because the number, ordering and sizes of runs per page will remain unchanged from our current simulation wherein freed memory and metadata are 0-tagged. This is because 
% speculate Results will remain the same.

\paragraphb{Prefetching Tags} MTE supports prefetching tags when cache lines are loaded for tagged memory. We can also support efficient pre-fetching of tags, with runtime similar to the {\sf LDG} operation, by also fetching information about neighboring runs when searching for a granule in the tree.
% Pre fetching tags can be done efficiently (O(depth) time)

\paragraphb{Page Swapping} When swapping pages in/out of the disk, the 128-byte buffer corresponding to the page being swapped (containing BTree or tag array) can be copied to/from the disk, along with the page.

% \paragraphb{Shared Memory} Potential AC attack but limited only to processes using pages with shared memory.

\paragraphb{Supporting Large Pointer Tags} Our design allows us to use much larger tags with limited memory usage. But, we are still limited by the size of the pointer tag. Currently, ARM supports TBI~\cite{linux-tag-addr-abi}, allowing the top 8 bits of pointers/virtual addresses to be used to store tags or other metadata. Also, Pointer Authentication Code (PAC)~\cite{arm-pac-whitepaper}, which was added to Armv8.3 for control flow integrity, is allowed to use the top 3-31 bits of the pointer, based on the processor's virtual address size.
% Four of these bits are used for MTE and the remaining 4 are used for PAC.
% But, we can currently use all 8 bits for memory tags only if PAC were turned off. 
To be able to use larger pointer tags for MTE, we could use all 8 bits in the top byte for MTE, or extend TBI to use some PAC bits for MTE. We discuss the possibility of combining MTE with PAC in \S\ref{sec:improve-combine-pac-mte}, to allow using up to 31 bits for memory safety.
We could also use the fat pointers idea wherein the tag is stored in another word and passed along with the pointer for address translation~\cite{cheri-isca14, lowfat-ptr}.

% Can allow using larger tags for both PAC and MTE, 

\paragraphb{Supporting LDGM/STGM for User space} Currently, bulk tag manipulation ({\sf LDGM/STGM}) instructions are supported only in kernel space. But our BTree design can do bulk tagging almost as efficiently as a single {\sf LDG/STG} call -- by getting/setting tags of a run (instead of a granule). Hence, it might be possible to support this instruction for user space as well.

\paragraphb{An attack: forcing pages to switch to a tag array} 
If an attacker could exploit a vulnerability and use techniques like heap grooming to cause a large number of runs on a single page, 
the system will switch that page to a tag array with short 4-bit tags.
Security for allocations on that page will be reduced to the security of current MTE, namely $1/16$ chance of guessing a tag. 
However, in a system that uses a randomized allocator~\cite{autoslab-heap-spray}, with features such as, (i) allocations are assigned random locations from the free list, (ii) separate blocks of memory for objects of different objects and/or sizes,
it can be difficult for an attacker to cause many runs on a single page.

% \paragraphb{Deciding tag sizes dynamically} TODO


% Not so easy. Also, this could be partially circumvented by periodically updating the secret key: issue, would need to re-tag all current ptrs, not good.
% Security analysis: compare MTE with PAC+MTE.

% A combination of PAC and MTE.   Can combine the bits for both into one block of eight bits. 

% One key $k$ for a pair-wise indep. hash stored in protected tag memory.  
% We need a data structure in every block, that let's us translate an address in the block 
% to the allocation number in the block.
% If we have such a data structure then tag storage is nothing, but we need to store the data structure.
% And we need to store 4-bits per pointer:  tag value (4 bits). 

% The tag for granule at address $a$ is 
% \[  t \gets H(k,(\text{page number},a_0, r)) \in \{0,1\}^4  \]
% where $a_0$ is the allocation number for address $a$ in the block and $r$ is the random tag generated at allocation. 
% In the pointer we store $t \in \{0,1\}^4$. 
% Now, the attack probability is $1/16$, as before, but page storage is just the data structure.  No tags.

% The point is:  if a pointer $p$ to buffer $A$ is incorrectly used to read from adjacent buffer $B$, then the computed tag
% for $p$ will be different than stored tag in the pointer $p$ with prob $1/16$,
% Because $b_0 \neq a_0$.   ($b_0$ is the allocated number of $B$)
% Discussion: kr,a0 OR kr,a OR kr,pg_num OR k,a0.

% which we write in the mem reserved for tag arr 
% e.g. [12bits pointer tag, 4bits same as tag array, 4bits to choose which seed, 4bits to match to OP of seed] : we have 8bit security by storing only 4bit tags + 16 seeds. Plus BTree for allocation starting granule.

% Per page seed. an attacker cannot attack other processes.

% \subsection{Storing Type information}. 
% TODO
% Moved to related work.

% \subsection{Re-tagging at type casting?}
% TODO
% Old pointers of a different type will not work anymore. : not ideal. (a compiler could do this too)


==> eurosp2023-template/intro.tex <==
\section{Introduction}

Memory corruption vulnerabilities continue to be the most widely reported class of vulnerabilities.
A report from the Google Chromium team~\cite{chromeSec} that examined 
%% https://www.chromium.org/Home/chromium-security/memory-safety/
912 high or critical severity security bugs since 2015 found that 
about 33\% are due to {\em spatial} bugs, such as buffer overflow, and
about 36\% are due to {\em temporal} bugs, such as use-after-free.
In response, an array of techniques have been deployed to make these vulnerabilities harder to exploit:
non-executable pages~\cite{ms-DEP}, 
address space randomization~\cite{ASLR}, 
stack canaries~\cite{canaries}, 
guard pages,
address sanitization~\cite{asan-atc-12,kasan-desc}, 
control flow integrity~\cite{CFI}, 
and many others. 

In addition to software techniques, 
processor companies have introduced architectural features to defend against memory corruption attacks,
such as a shadow stack and EndBranch in Intel CET~\cite{cet}. 
ARMv8.3 added support for cryptographic control flow integrity~\cite{ccfi}.
This feature, called ARM Pointer Authentication Codes (PAC)~\cite{arm-pac-whitepaper},
embeds a short (say, 16 bits) cryptographic integrity code (MAC) in the top bits of every 64-bit function pointer and return address.  
The MAC is checked before the pointer is dereferenced and an exception is raised if the MAC is invalid.
While this feature ensures that a pointer cannot be overwritten with an arbitrary value~\cite{pac-parts-sec19},
it cannot enforce memory safety. 

%works well for function pointers~\cite{pac-parts-sec19},
%it is more difficult to use for data pointers because it prevents pointer arithmetic,
%as commonly used to reference array elements.

ARMv8.5 recently added an important mechanism, called Memory Tagging Extension (MTE)~\cite{arm-mte-whitepaper},
to improve the memory safety of code written in an unsafe language, while requiring no source changes. 
%It can be used to detect some buffer overflows, use-after-free, double free,
%and other memory corruption bugs. 
MTE implements a tagging approach to memory access, as proposed in \cite{mem-tagging-google}.
The design is closely related to the design of Hardware-assisted AddressSanitizer (\href{https://clang.llvm.org/docs/HardwareAssistedAddressSanitizerDesign.html}{HWASan}). % Android's 

MTE has two parts.  First, all of physical memory is divided into 16-byte granules, and each granule is given an associated 4-bit tag.
These tags are managed by the hardware and are stored in a reserved location in RAM.  
For example, for 64GB of physical memory, the tags take up 2GB of space. 
Second, every pointer and virtual address is modified to contain a 4-bit tag in its top byte. %, using the Top Byte Ignore feature of Arm~\cite{arm-mte-blog}. 
This is possible in a 64-bit system because the top byte of a pointer is not used for address translation.
When a pointer is used to access memory, the hardware first verifies that the 4-bit tag embedded in the pointer
matches the 4-bit tag associated with the 16-byte granule being accessed.  
If not, the hardware raises an exception or records that a mismatch occurred.
The reason for using 16-byte granules is explained in~\cite[p.\@ 6]{mem-tagging-google}:
larger granules reduce tag storage, but harm the security of MTE and cause other overheads due to alignment requirements.

\smallskip\noindent
Let us briefly look at a few applications of MTE:
\begin{itemize}%[leftmargin=1em,itemsep=1ex]
\item
MTE can reduce the likelihood of a buffer overflow by ensuring that consecutive buffers are tagged with different 4-bit tags.
That way, a pointer into one buffer will trigger an exception if it tries to write to an adjacent buffer.
\item 
MTE can reduce the likelihood of a use-after-free by enhancing the {\tt free} function to change the 4-bit tags associated
with all the granules being freed.  
A dangling pointer will then trigger an exception if it tries to read from or write to the freed space.
\item
MTE can reduce the likelihood of a double-free by making the {\tt free} function check
that the tag in the given pointer matches the tag of the granules being freed, and do nothing if not. 
Since {\tt free} changes the tags of the freed granules, freeing the same space again will do nothing.
\end{itemize}
We stress that these protections are not foolproof and discuss this further
in Section~\ref{sec:usage-survey}.

\smallskip
In Section~\ref{sec:overview} we review the hardware features of MTE 
as well as the Linux kernel changes that were needed to support MTE.
We fill in some details that are missing from ARM's description.


\paragraphb{Our contributions}
Memory allocators need to be modified to take advantage of MTE:
{\tt malloc} needs to tag newly allocated memory and {\tt free} needs to change these tags.
We examined the allocators used in a number of projects and found 
that every project chose to implement a different tagging strategy.
In Section~\ref{sec:usage-survey} we survey the tagging strategies used by 
Glibc, Android Scudo, Linux Slub, Chrome, and LLVM (for tagging stack granules).  

We found significant differences between the tagging strategies in the projects listed above. 
While all of these projects benefit from using MTE, 
some of the strategies used offer much weaker protection than what can be achieved using MTE.
We describe some potential vulnerabilities in all five allocators, 
and describe ways in which the security of these allocators can be improved
with relatively inexpensive modifications. 
We note that currently, there is no support for MTE in iOS, Windows, and the Go runtime.

\smallskip
\paragraphb{Improving MTE}
Next, we look at improving the design of MTE.  
MTE uses 4-bit tags which means that an attacker can guess a required tag with probability $1/16$.
While pointers can accommodate larger tags, the reason 4-bit tags are used is due
to the space required to store tags: 2GB of memory is needed to store tags for a system with 64GB physical memory.
Larger tags, say 16-bit tags, would quadruple the required memory.

In Section~\ref{sec:improvements} we propose a way to support larger tags, 
but without increasing the required memory to store tags.
Our observation is that many allocations are comprised of multiple consecutive granules
{\em where all granules have the same tag}.
This means that we can compress the set of tags using run-length-encoding
and only store the starting point of an allocation, the number of granules it contains, and the assigned tag.
There is no need to store all the tags associated with the allocation in an explicit tag array.
The challenge is that allocations are constantly malloc'ed and free'ed and we need
a data structure that can handle a dynamic run-length-encoding with a fast lookup and a fast update.
We describe such a data structure in Section~\ref{sec:improvements}.
As an additional benefit, this data structure makes it possible to set the tag of many granules at once, 
which can improve the performance of malloc and free.

Next, we implement a modified version of MTE using our data structure.
Our implementation is a software patch to QEMU's emulation of ARMv8.5.
The result is an ARM emulator that implements our modified MTE.

We then experiment with several applications to measure the space savings in tag storage due to our modified MTE.
We experiment with Apache2, md5, FFmpeg, pbzip2, and axel.  
The space savings are significant in applications that mostly make large allocations
and more modest in applications that predominantly make small allocations. 
Figures~\ref{fig:workloads-avg} and~\ref{fig:workload-alloc-cdf} describe the distribution of allocation sizes for each application we experimented with.
%They show that md5 has the smallest average allocation size of these workloads. 
Our detailed evaluation in Section~\ref{sec:btree-storage-eval} shows that for all the applications 
we tested, our design supports large tags, even 32-bits long, for 58\% to 99.9\% of RAM (depending on the application) 
with the same storage as MTE's current implementation. 

To summarize, our experiments show that we can support larger tags, 
8, 16, and even 32 bits per granule, for most of RAM, with the same memory overhead for tag storage
as the current implementation of MTE.
The cost is a more complex data structure than the simple tag array used in the current MTE.

Recall that MTE tags are stored in the high-order bits of every pointer,
and this space is also used by PAC (pointer authentication). 
In Section~\ref{sec:additional} we discuss unifying PAC and MTE into a
single value stored in the high-order bits of every pointer.  
We show that this provides protection equivalent to the combination of 16-bit MTE and 16-bit PAC, while only using 16-bits in the pointer.
%compared to two standalone implementation of PAC and MTE. 
Finally, we discuss related work in Section~\ref{sec:related}.











\ignore{
\paragraphb{Consequences}
We enable tags to become 8 -- 16 bits per granule instead of 4 bits per granule. 
Note: currently, setting the tags for an entire page is so expensive that scudo (secondary alloc) doesnt use tagging for large allocations. With a BTree, this operation would be as cheap as setting the tag of 1 granule.
However, this requires more space in every pointer.  
So, either we have to use shorter PAC or we need to rely on fat pointers. 
Cite performance analysis of fat pointers. 
We can even support 16 bits tags, but that might eat up more memory per page. 
}




%In this work, we first present a survey of memory tagging implementation across various memory allocators and compilers, and demonstrate simple exploits on glibc and Clang-LLVM. Second, we list potential improvements to MTE, namely a. Defining invalid tags to enhance use-after-free detection, b. Using RLE-encoding to reduce the memory overhead of MTE by compressing the tag storage. Both together will strengthen MTE's security guarantees
% which will allow us to use larger tags (and hence stronger security) 
%while using same or lesser memory.




% C and C++ have been, and still are one of the most popular languages - a huge amount of code in-use today is written in these languages, with Debian Linux alone containing more than half a billion lines \cite{deb-linux-loc, arm-mte-blog}.

% % [mem safety - types of attacks, stats]
% The languages, while being well known for their performance and flexibility, do not provide memory safety. 
% Accessing memory out-of-bounds (e.g. buffer overflow), or use-after-free or uninitialized memory are some of the memory safety bugs
% % Buffer overflows, use-after-free, out of bounds, use after free, using uninitialized memory etc, 
% , that can lead to attackers getting access to sensitive data and/or remote code execution. 
% Such memory safety bugs are the largest portion of security vulnerabilities. Nearly 70\% of all security issues addressed in Microsoft products are caused by memory safety violations \cite{ms-mem-viol}. Similarly, over 75\% of vulnerabilities found in Google's Android are based on memory unsafety \cite{google-mem-viol}.
% % : microsoft - 60\% , 
% % Google Android: 75\% vulnerabilities are memory safety  
% % , 60\% of Project Zero bug reports are mem corruption attacks.
% % control over the program and calling ?....

% There has been a lot of research in building tools to detect such memory bugs in both testing and production environments. Address sanitizer (and hardware assisted address sanitizer) \cite{addsan-ms, san-for-sec-sok} is a widely used tool
% % , which uses compiler instrumentation to observe all memory load and store instructions, 
% to detect bugs at runtime, but can only be used for testing due to its huge memory and performance overhead. Fuzz testing \cite{google-fuzz} is another tool for security testing, but it cannot catch all possible bugs. 
% % No-FAT is a recent technique that uses binned memory allocators

% Code hardening techniques, such as stack canaries \cite{ms-stack-canary}, non executable memory \cite{ms-DEP}, ASLR, control flow integrity (LLVM CFI \cite{llvm-cfi}, Microsoft CFG \cite{ms-cfg} and Shadow Call Stack, Intel CET) and pointer integrity (ARM Pointer Authentication, PARTS \cite{parts}) all help prevent memory safety bugs from hijacking control flow. While all these tools make control flow attacks much harder, they do not solve memory exploitation, which is the root cause of most of these attacks.

% % [existing work : in testing and in production] lots of work - ASan, fuzzing during testing. but too slow to run in production. 
% Memory tagging is a hardware based memory safety solution, that implements a lock and key based access to memory - locks can be set on allocation (for each memory location and stored in memory), and the correct key must be provided for accessing memory. SPARC ADI and ARM MTE \cite{arm-mte-blog} are both based on memory tagging in hardware. Google has adopted Arm's MTE in Android \cite{google-android-mte} due to its low performance and memory overhead. 
% % [todo: add 1. survey & exploits, 2. improvements]

% While MTE seems like a promising solution, using it requires changes across the stack - the kernel, compilers and memory management libraries need to be aware of MTE and tag memory accordingly. Also, both SPARC ADI and ARM MTE suffer from restricted security guarantees (small tags), which they trade off to reduce the memory overhead of storing the tags for all memory locations. While there have been recent works to achieve a better memory - security trade-off, specifically No-FAT \cite{nofat-isca-21} and CrypTAG \cite{cryptag-arxiv}, they suffer from limited safety against temporal memory attacks (i.e. use after free) and large cache overheads respectively.
% % maintain a low memory overhead by reducing their security guarantees 

% % Mem taggin - SPARC ADI, ARM MTE : , Google has . While great, security limited to 4 bits of the tag - due to overhead of storing the tag of every single granule in memory.

% % No-FAT and CrypTag? : attempts to improve MTE.



==> eurosp2023-template/mte-background-new.tex <==
\section{Overview of Memory Tagging}
\label{sec:overview}

We begin by describing the detailed operation of MTE
at both the hardware and kernel levels. 
Our description fills in some details that are not described in the
MTE whitepaper~\cite{arm-mte-whitepaper,arm-mte-blog}.

\subsection{Architectural Changes} 

\paragraphb{Memory \& Cache Changes} MTE adds a new memory type called Normal tagged memory. A global tag array stores a 4-bit tag for every 16 bytes (granule) of this memory type: for example, for a machine with 64GB of tagged RAM, the tag array would require 2GB. These tags are stored either in RAM reserved by firmware or in the metadata space available in DRAM chips such as ECC bits. Tags are pre-fetched when cache lines are loaded for tagged memory.  There is also a tag cache used for caching tags. 
Note that tags are applied to physical memory, not to virtual addresses.
%A shared memory page between two processes will always have the same tag,
%even if it is mapped to a different virtual address in each process.

\paragraphb{ISA Extensions} MTE adds new instructions for handling tagged memory. 
For every load and store to a granule in tagged memory,
the hardware compares the tag in the top byte of the address register to the tag assigned to the granule being accessed, and can raise an exception in case of mismatch. The {\sf LDG} and {\sf STG} instructions are used to get and set the tag of a granule. The instructions {\sf LDGM} and {\sf STGM} do bulk tag manipulation, but can only be used by system software at Exception Level 1 or higher (e.g. the kernel). These instructions load/store the tags of 1 to 16 consecutive granules at once. %The register {\sf GMID\_EL1.BS} controls the exact number of tags that will be read/written.

The {\sf ADDG} and {\sf SUBG} instructions are used for pointer arithmetic: they modify the tag and address separately by an immediate value. 
The {\sf IRG} instruction is used to generate a random tag for a granule. 

% are done via new instructions, such as LDG, STG. [1line ldg-stg+1line ldgm, 1line addg-subg, 1line irg]
% LDG/STG instructions have been added for getting/setting the tag for a single memory granule.

% \begin{itemize}
% % 	\item  New memory type : normal tagged memory. Where are tags stored (for 64GB RAM, 2GB:  RAM is reserved or ECC bits are used for tag memory) 
% % 	\item Tag Cache: There is also a separate cache for storing tags. Pre-fetching.
% % 	\item TODO: who calls LDG? does LDR call LDG?
% % 	\item Loads and stores to this memory are done via new instructions LDG, STG: ,
% % 	STZG, LDGM/STGM - 
% % 	loads and stores to this new memory type perform an access where the tag present 
% % in the top byte of the address register is compared with the tag stored in memory
% % the tag in the pointer is compared to the tag of the memory being accessed. Tags are pre-fetched. 
% % 	\item IRG: insert random tag, 
% % 	\item Tag \& Pointer arithmetic: such as addg/subg.

% \end{itemize}

\paragraphb{Tag Checking Controls}
MTE defines new system registers that control tag-checking behavior. 

\paragraphi{Global control} The \href{https://developer.arm.com/documentation/ddi0595/2020-12/AArch64-Registers/TCO--Tag-Check-Override}{{\sf TCO}}  register (Tag Check Override) can be used to disable all memory tag checking. Setting the 25th bit of this register to 1 disables tag checking for all loads and stores to tagged memory.

\paragraphi{Handling tag mismatches} When tagging is enabled, there are two modes for handling tag mismatches: synchronous, wherein the hardware throws an exception on tag mismatch; and asynchronous, wherein the CPU accumulates tag mismatch information in a system register ({\sf TFSR\_ELx} or {\sf TFSR\_EL1} for user mode)~\cite{linux-mte-async}. 
In asynchronous mode, the kernel can react to tag faults 
during a context switch or a system call, 
for example, by killing the offending process or thread.
This mode has a lower performance overhead but is less precise than 
synchronous mode. 

\paragraphi{The match-all tag} MTE provides the option of using {\tt 0xF} as a match-all tag, in kernel space. Specifically, if the TCMA bit of the translation control register (\href{https://developer.arm.com/documentation/ddi0595/2020-12/AArch64-Registers/TCR-EL1--Translation-Control-Register--EL1-?lang=en\#fieldset_0-58_58-1}{{\sf TCR\_EL1}}) is enabled, then all memory accesses from EL1 (kernel space), using a pointer tagged with {\tt 0xF}, are not checked for tag equality. This feature is likely inherited from the match-all tag in the software-based kernel address sanitizer (\href{https://www.kernel.org/doc/html/latest/dev-tools/kasan.html}{KASAN}).
It lets the kernel allocate a large buffer, 
without spending the time to set the tags 
for all the granules in the buffer. 


\subsection{OS/Kernel Support}

The Linux kernel added support for enabling memory tagging. 
We describe the key updates to the kernel.

\paragraphi{Enabling tagged addresses} 
To enable MTE, a user process must 
call {\rm prctl} with the {\sc pr\_set\_tagged\_addr\_ctrl}
option to be able to pass tagged addresses to the kernel~\cite{linux-prot-mte}.
It must also enable the tagged memory attribute on an address range using a new {\sc prot\_mte} flag for the mmap and mprotect functions. 
These flags must also be set for stack pages when the process starts, to enable tagging for the stack. The tags are initially set to 0 whenever a page is mapped to a process' memory, and preserved on copy on write. 
Clearing tags for a new page is necessary to avoid leaking sensitive information about the previous owner of the page. 
%This is similar to the issue pointed out in this paper~\cite{garbage} which %%forces the OS to clear the contents of a physical page
% once it is released by a process.
% new process : tags reset to 0 for allocated pages, mte disabled by default.
% Whenever a page is allocated to a process, the OS resets the tags to 0.

\paragraphi{Configuring tag mismatch behavior} The tag checking mode (synchronous or asynchronous) is selected for each process by calling prctl with the corresponding flag. Tag mismatches are ignored if no mode is specified.  If a thread's checking mode is none or asynchronous, then kernel accesses to user space are not checked for a matching tag. If the mode is synchronous, the kernel makes a best effort to check its accesses to user space~\cite{linux-prot-mte}.
% Todo: Maybe add per cpu preferred tag check mode?

\paragraphi{Forking} When a process forks, the child process inherits the parent's tagging configuration, memory map attributes, and the memory tags.

\paragraphi{Shared Memory} Linux supports using both {\sc map\_shared} and {\sc map\_private} with MTE, but 
%only with {\sc map\_anonymous}, i.e. 
tagging is not supported for file-backed memory mappings. With {\sc map\_shared}~\cite{linux-prot-mte}, both memory and its corresponding tags can be shared between processes. Interestingly, if a process shares memory with a forked child using {\sc map\_shared}, 
and the child changes a tag assigned to shared memory, then the parent's pointers to that address will no longer function. 
%then memory tagged by a child process after forking will not be accessible by the parent, since only the child will have a properly tagged pointer.
% both shared and private mmap are supported, but only with map\_anonymous. Memory (and corresponding Tags) can be shared b/w processes using MAP\_SHARED.


\paragraphi{Supporting ptrace} Linux has added support for a tracker process to read and write tags of another process using ptrace, with requests 
{\sc ptrace\_peekmtetags} and {\sc ptrace\_pokemtetags} respectively.

\paragraphi{Page Swapping and Hibernation} A new page flag has been added to track whether a page
has been mapped into user space with MTE enabled. 
The tags are saved/restored when the page is swapped out/in respectively. 
Hibernation support uses the same page flag to copy tags out of tag storage and into memory before the hibernation image is created~\cite{linux-mte-page-swap-hibernate}.
Similarly, Linux has added support to save/restore system registers, such as {\sf TFSR\_EL1}, during suspension~\cite{linux-mte-async}.

\subsection{MTE Limitations}
While MTE is a powerful low-overhead approach to memory safety, it does not prevent all memory corruption attacks.
In particular, it does not protect against:

\paragraphi{Intra-object overflows} When an object is allocated, memory for all its sub-fields is tagged with the same value, so that the returned pointer can be used to access the entire object.  Consequently, an intra-object overflow can be used to corrupt data and pointers contained within the object without causing a tag mismatch exception.

%%%  this is not quite a memory corruption attack
%\paragraphi{Type errors} MTE provides no protection for attacks based on type errors, e.g. an object of one type being incorrectly interpreted as an object of a %different type (allowing object 
%fields to be accessed and used incorrectly).
%We do note that most type confusion attacks use spatial/temporal unsafety as the first primitive, meaning they can be avoided with %MTE~\cite{msrc-mte-secu-analy}.

\paragraphi{Blind ROP Attacks} One could attack an MTE-based server in a similar fashion to the Blind ROP attack~\cite{brop-hacking-blind}, 
namely determining the tag of a memory granule, by trying multiple guesses and checking if the server crashes and re-starts. 
Since tags are only 4 bits, this will take 16 restarts in expectation. 

\paragraphi{Speculative execution} Attacks based on speculative execution (such as Spectre~\cite{spectre}) could be used to infer the memory tag value of a granule without triggering a tagging violation~\cite{nofat-isca-21}.

These weaknesses have also been pointed out in past works~\cite{tag-guide, msrc-mte-secu-analy, msrc-bluehat-mte-attack}.
% TODO: perhaps mention no invalid tag. Then in Section 5 talk about adding an invalid tag.


==> eurosp2023-template/related-work.tex <==

\section{Additional related work}
\label{sec:related}

In this section we review more of the related work relating to address sanitization and memory tagging. 

Address Sanitizer (ASan)~\cite{asan-atc-12} is a software-only tool based on compiler instrumentation introduced to the LLVM and GCC compilers in 2011. It uses red-zones around every object for spatial safety, uses quarantines to delay the reuse of freed objects to detect temporal bugs, and also stores 1-byte metadata per 8 bytes of memory to mark memory as valid/invalid. While ASan is heavily used in testing, it cannot be used in production code due to its large CPU and RAM overhead.
Califorms~\cite{califorms-micro19} is a research proposal based on the idea of blacklisting freed memory and memory around allocations, similar to ASan's quarantine and red-zones. This has a high overhead and also cannot protect against non-linear overflow beyond the blacklisted memory. 
MarkUs~\cite{markus-sp20} uses an approach similar to quarantines, but provides no safety against spatial attacks. 

%\href{https://clang.llvm.org/docs/UndefinedBehaviorSanitizer.html}{UBSan} is a fast undefined behavior detector, which modifies the program at compile time. It detects buffer overflows where the bounds can be statically determined, and hence provides limited protection.

There is considerable prior work on storing metadata to enforce memory safety. 
Fat pointer schemes that maintain such metadata in a separate memory region~\cite{hardbound-asplos08, softbound-pldi09, intel-mpx} incur a large CPU and memory overhead. 
%BOGO~\cite{bogo-asplos19} is based on top of Intel MPX, but LLVM and GCC have already dropped support for Intel MPX in their mainline due to its high overheads.
CHERI~\cite{cheri-isca14} is a popular proposal that stores metadata inline with the pointer.  However, it changes the memory layout and loses pointer-size compatibility with legacy code.

In-FAT pointers~\cite{infat-asplos21} provide both inter and intra-object spatial safety using per pointer metadata, but cannot protect against temporal attacks. FRAMER~\cite{framer-acsac19} uses 16-bit pointer tags to lookup object metadata stored near each object, but has large performance overheads due to its software-based implementation. Low-FAT pointers~\cite{lowfat-ptr, lowfat-ptrs-stack} use binned allocators and store the size of the object within the pointer to provide spatial safety, but they have large memory overheads with no temporal safety. CUP~\cite{cup-asia-ccs-18} is another approach that uses the entire pointer to store tags to index into a metadata table storing base and bounds. However, this only provides partial temporal safety and also has a large performance overhead, since the pointer first needs to be translated into an actual address before it can be de-referenced.

AOS~\cite{aos-micro-20} stores a pointer authentication code (based on PAC~\cite{arm-pac-whitepaper}) in the pointer's top bits, and uses it to index into a hash table storing object bounds. It provides partial temporal safety and does not apply if external (unmodified) modules modify a pointer. 
% \aditi{Here}
PACSan~\cite{pacsan-arxiv} uses a similar idea, it generates a pseudo-random birthmark when an object is allocated (similar to MTE tags) and uses a PAC code to index into a hash table that stores the birthmark and object bounds. But it is susceptible to use-after-realloc (UAR) because the birthmark is not fully random. It also does not support tag caching, pre-fetching, and page swapping.
% if an attacker allocates another object of the same size, when the stack pointer is the same.

There is considerable work on memory tagging. \href{https://clang.llvm.org/docs/HardwareAssistedAddressSanitizerDesign.html}{HWAsan} is a compiler-based tool, that uses 8-bit tags for every 16 bytes of memory. But since it adds extra instructions to check tags before every memory access, it has a $2\times$ performance overhead. The Generic and Software-Tag modes of \href{https://www.kernel.org/doc/html/latest/dev-tools/kasan.html}{KASAN} also use compile-time instrumentation to enforce memory safety using shadow memory, quarantine, and memory tagging.  
UAFSan~\cite{uafsan-issta21} generates a tag at each allocation/de-allocation and stores the tag as metadata for each object and pointer. 
It has considerable memory and performance overhead, and only handles temporal safety. 
All these compiler-instrumentation based tools require re-compilation of source code.

No-FAT pointers~\cite{nofat-isca-21} combine memory tagging with Low-FAT pointers to get temporal and spatial safety. But, 
% its temporal safety when pointers are passed to functions is unclear, and,
both No-FAT and Low-FAT require pointers to be within bounds when passed to functions, which is too strict for real-world programs.
CrypTAG~\cite{cryptag-arxiv} combines tagging and encryption -- it stores the tag in the pointer, but, instead of storing the tag for every granule in memory, it encrypts data with the tag as additional input for encryption. % Their scheme requires a hardware encryption unit to be practical and also has huge cache overheads.

\cite{msrc-mte-secu-analy} analyses the security of MTE, and recommends that adjacent allocations always have different tags. \cite{msrc-bluehat-mte-attack} discusses a potential attack on MTE, but it is based on the assumption that there is no re-tagging on free; 
this is not the case in the applications we surveyed in Section~\ref{sec:usage-survey}. %Hence, their attack would only work with a small probability in real-world scenarios.
~\cite{tag-guide} presents a survey of tagged architectures and challenges in deploying MTE in the real world. 
While all these works point out issues with MTE, they do not explore the security of software systems using tagging (Section~\ref{sec:usage-survey}) or implementation improvements to MTE,
as in Sections~\ref{sec:improvements} and~\ref{sec:additional}.

HAKC~\cite{hakc-ndss-20} also uses both PAC and MTE to achieve kernel compartmentalization, which is orthogonal to our work. We instead combined them to achieve both memory safety and pointer integrity while using a single 16-bit tag.

MTE does not protect against type errors, and as such, the work on type checking~\cite{effective-san, typesan-ccs16} is complementary to and can be used in conjunction with MTE. 
% Todo: type checking: 
% EffectiveSan, TypeSan. Mention that Since the BTree allows us to store tags in much smaller space, we can use larger tags, and also store type information within the tag.
% Similar to LLVM TySan.

%Prior work on control flow integrity, such as~\cite{arm-pac-whitepaper, pac-parts-sec19} and \href{https://developer.arm.com/documentation/ddi0602/2021-12/Base-Instructions/BTI--Branch-Target-Identification-}{ARM BTI}, 
%is orthogonal to memory safety and can be used in conjunction with MTE. 
% As discussed in \S\ref{sec:improve-combine-pac-mte}, we could combine PAC and MTE for data pointers to enhance security.
% TODO:  PAC on Armv8.3A and Armv8.1-M (32bit, PAC stored in GPR register)
% PARTS : based on ARM pointer auth 
% , Intel IBT, ARM BTI, PAC Security'22 paper


% .\subsection{Sanitizers}
% ASan (uses 1byte tag per 8bytes of memory, redzones for buffer overflow detection, quarantines for detecting use after frees), UBSan

% \subsection{Control Flow Integrity}
%  CFI tries to restrict the control-flow of a program to valid execution traces. e.g. Stack canaries and shadow call stack are techniques to detect if the return address of a function has been corrupted. Other techniques such as LLVM CFI, Microsoft CFG, ARM Pointer Authentication, DEP try to avoid corruption of function pointers etc, by placing tight restrictions on where an application can execute code from. While these tools are effective at making arbitrary code execution hard, they do not solve the main root cause of such exploits i.e. memory corruption itself \cite{sok-war-mem}.
 




% TODO: AOS (use PAC to index into a per-process hashed bounds table), UAFSan (use after free San), DangKiller, CHERI (capability based)

% \subsection{Memory Tagging}

% \paragraphb{No-FAT} Memory tagging + binned allocators, tagging + LowFat, Potential temporal/spatial attacks: esp over function calls.

% \paragraphb{CrypTAG}. 
% Combines tagging and encryption, wherein it stores the tag in the pointer, but, instead of storing the tag for every granule in memory, it encrypts the value stored with the tag as additional input for encryption. This alows them to use 25-bit long tags. Their scheme requires a hardware encryption unit to be practical, and also has huge cache overheads since they store both the decrypted value and the (long) tag in cache.

% \paragraphb{KASAN}. Generic and S/W KASAN.

% \paragraphb{HWAsan}~\cite{hwasan-android, hwasan-clang}. for every allocation, a random tag is assigned to the pointer and to memory (tag stored separately for every granule, in an array in shadow memory). For short allocations, tag is stored in last byte of granule and shadow memory stores the size of the allocation.
% Possible attack:  if size of an allocation is known: use tag == size? (since tag=size will match ptr tag, no exception?), will be able to load/store the data.

% TODO: MSRC paper (analysis, recommends adjacent allocations always have different tags). They discuss an attack on MTE, but that is based ont he assumption that there is no re-tagging on free - we have observed this is not the case in all the applications that we surveyed. Hence, their attack would only work with some small probability. [Their attack would work with probability only (1/16)\^2 if memory is re-tagged on free (i.e. random on malloc, re-tag on  free)]

==> eurosp2023-template/usage-survey.tex <==
\section{How MTE is used in Real-World Systems}
\label{sec:usage-survey}

Next, we look at how software systems have adapted to use memory tagging.
Every project uses a different strategy for implementing tagging,
and we review the security of these variants.

%In this section, we present a survey and security analysis of how various memory allocators and compilers have
%implemented tagging for heap and stack variables. 
% We believe our survey to be representative since it covers most common allocators used in C++ code, in popular OSes such as Linux, Android and in Chrome which is a popular browser, as well as LLVM, which is the back-end 

%%  Five subsections
%%  Explain how MTE is used in glibc, Linux, Chromium, Android, LLVM
%%  For each one, explain how MTE is used on the heap and how it is used on the stack.
% mark pointer and memory with the chosen tag value
% On each memory allocation, we can generate a random tag, embed it into   the returned pointer and set the memory tags that correspond to this chunk of memory to the same value.

\input{usage_survey_files/glibc}
\input{usage_survey_files/linux}
\input{usage_survey_files/scudo_android}
\input{usage_survey_files/chromium_ptalloc}
\input{usage_survey_files/llvm_stack}

% [random tag on allocation, increments tag by 1 on free]


\ignore{
\begin{table*}[]
\begin{center}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
Appl.
& \begin{tabular}[c]{@{}l@{}}Spatial\\Linear \\ Benign \end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Spatial \\ Linear \\ Malicious \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Spatial \\ Non-Linear \\ Benign \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Spatial \\ Non-Linear \\ Malicious \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Temporal \\ Use-after-free\\ Benign \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Temporal \\ Use-after-free\\ Malicious \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Temporal \\ Use-after-realloc\\ Benign \end{tabular}
& \begin{tabular}[c]{@{}l@{}}Temporal \\ Use-after-realloc\\ Malicious \end{tabular}
% Application & \multicolumn{2}{c|}{Adjacent Overflow} & Non-adjacent Overflow & Use-after-free & Use-after-realloc 
\\ \hline

glibc & 100 & 0 & 93.7 & 93.7   & 100 & 0 & 93.3 & 93.3  \\ \hline

Chrome & 93.7 & 93.7 & 93.7 & 93.7 & 100 & 0 & 100 & 0  \\ \hline

\begin{tabular}[c]{@{}l@{}}Scudo\\ (Primary) \end{tabular}       &   100 & 0  & 93.7 & 93.7  & 87.5 & 87.5 & 87.5 & 87.5 \\ \hline

Linux SLUB  &     92.9 & 92.9 &  93.3 & 93.3    &  100 & 0  &  92.9 & 92.9                \\ 
\hline
\end{tabular}
}
\vspace{10pt}
\caption{\rm Summary of protection of surveyed libraries against common spatial and temporal attacks. We list the probability of detection of each attack (in \%). 
We are assuming that allocations have no extra granules in Linux and that the odd-even feature is turned on for Scudo.}
\vspace{-20pt}
\label{tab:survey-sec-summary}
\end{center}
\end{table*}
}


\ignore{
\subsection{Summary}
Table \ref{tab:survey-sec-summary} summarizes the security analysis of the tagging behaviors of all the libraries that we surveyed. 

To summarize, it is important to tag memory with a random value at every allocation/de-allocation, since any deterministic tagging behavior can lead to attacks as seen in \S\ref{sec:mte-impl-glibc}
 - \ref{sec:mte-impl-llvm}. 
 
 At de-allocation, choosing a random tag different from the allocation's current tag can help protect against benign Use-after-frees deterministically, help detect double free's by comparing pointer and memory tags, and protect against malicious Use-after-frees with probability 93\% (or 87\% if Scudo's odd-even feature is used).
 
To protect against attacks on internal metadata, the granules containing  metadata should be tagged randomly. A checksum of the metadata can also be stored for detecting corruption, similar to Scudo (\S\ref{sec:mte-impl-scudo}). 
 
Scudo's odd-even feature improves protection against benign buffer overflows, at the cost of lowering detection probability for temporal attacks from 93\% to 87\%. We propose an alternate approach - for every allocation/de-allocation/metadata, we generate a new random tag, out of 14 possible values, excluding the tags of granules on both sides. This might be less efficient ({\sf LDG} might need to be called to get neighboring tags), but it provides deterministic protection against benign buffer overflows, and  only slightly lowers the detection probability for temporal attacks to $13/14$ (1 in 14 chance of random match), i.e. 92.8\%. Hence, this approach achieves stronger security than the odd-even feature.

}
% odd even tag improvement
 
% \begin{table*}[htbp]
% \caption{Summary of how MTE is used in Real World Systems}
% \begin{center}
% \begin{tabular}{|c|c|c|c|}
% \hline
% Appln & At Allocation & At Deallocation & Metadata \\ \hline
% Glibc & Random tag & Zero tag & Zero tag \\ \hline
% Linux SLUB & Random tag & Invalid tag (0xE) & ? \\ \hline
% Chrome PartitionAlloc & Random & Increment by 1 & ? \\ \hline
% Android Scudo & Random & Random & Checksum \\ \hline
% \end{tabular}
% \label{tab-usage-survey}
% \end{center}
% \end{table*}

% \subsection{Global Variables Tagging}
% Todo. Need compiler support.



% \subsection{Resetting tags}
% [Moved to mte overview]
% {\bf TODO:} explain that the OS must reset all tags on a physical page prior to mapping the page to the virtual address space of a user space process.
% Otherwise, the residual tag values could leak information about what the previous owner of the page did.   This may leak password lengths and possibly
%  other value.  Confirm that Linux does indeed reset tags. 
 
%  This is similar to the issue pointed out in this paper~\cite{garbage} which forces the OS to clear the contents of a physical page
%  once it is released by a process.   The same reasoning requires the OS to clear all the tags from a physical page once it is
%  released by a process. 

==> eurosp2023-template/usage_survey_files/chromium_ptalloc.tex <==
\subsection{Chrome PartitionAlloc}
\label{sec:mte-impl-chrome}
PartitionAlloc is the heap memory manager used by both Chrome and Chromium browsers.
%, which occupy more than 70\% of the worldwide browser market share.
% Both Chrome and Chromium browsers use the PartitionAlloc for heap memory management.
This allocator splits memory into different partitions, each reserved for objects of a specific type or size.
Different partitions exist in different regions of the process address space, and there is a guard page on both sides of each partition. 

The allocator uses MTE tagging as follows: at every malloc call (i.e. new heap variable), it generates a random tag, which it assigns to all the allocated memory granules, and to the returned pointer. At free, it increments the tag by 1 for all the freed granules~\cite{chromium-ptalloc-mte}. When re-allocating previously freed memory, it re-uses the incremented tag, and simply assigns it to the returned pointer. 
This optimization improves malloc time. Larger allocations have guard pages on both sides.
%Allocations that are too big are served with a direct map and have guard pages on both sides.

%PartitionAlloc stores most of its metadata in a region separate from all the allocations. Free list pointers are stored in freed memory, but a shadow pointer is also stored to detect corruptions.
% The only metadata that is stored adjacent to objects are the free list pointers, which store the locations of free slots in a partition. These are stored at the beginning of each free slot. To detect corruption, the freelist pointers are stored in an encoded form.  

The chrome team implemented an interesting mechanism~\cite{chrome-security-blog-uaf-scan} on top of MTE to further defend against use-after-free. 
Their concern is that, due to the ``increment by one'' tagging strategy, 
an attacker can wait for 16 malloc/free cycles of a memory location until the tag for that memory cycles back to an old tag value.
A dangling pointer can be used at that time without triggering a tag mismatch exception. 
To prevent this they use quarantining: when the 4-bit tag of a memory location reaches zero, that location is placed in a quarantine list and is not re-allocated until a periodic heap scan checks that no dangling pointers are pointing to this location.
If so, the location is removed from the quarantine list and can be re-allocated.

%\paragraphb{Security} 
%We use the same threat model as used for glibc.
% c - the attacker has access to the application's source code and binary, and the attacker can craft pointers with arbitrary tags and addresses. For simplicity, we assume that the code has input-dependent pointer arithmetic, and the attacker can control the inputs to get desired tags and addresses.
\ignore{
\paragraphi{Spatial Safety} Adjacent and non-adjacent overflows are protected probabilistically.
% Both adjacent and non-adjacent overflows within the same partition, can succeed only with a probability of 7\%, since there's a 1 in 16 chance of the pointer tag randomly matching the memory tag. A malicious overflow attempt can also work with only 7\% probability.
Guard pages help detect overflows across partitions and across large allocations.
% Overflowing into a different partition can be caught deterministically if it falls onto the guard pages between partitions. Similarly for large allocations, overflow can be caught because of the guard pages adjacent to the allocation.

% random cuz no metadata bw allocs - for adj, non-adj, benign, malicious.
}

% \begin{lstlisting}[language=c, caption={test}, captionpos=b, label={lst:test}]
% void src_code(long delta, int val) {
%     char* arr1 = malloc(64);
%     char* arr2 = arr1;
%     free(arr1);
%     // arr2 is now a dangling pointer
%     char* arr3 = malloc(64);
%     // delta:
%     int delta = arr3 - arr1;
%     //  
% }

% \end{lstlisting}


\ignore{
 \begin{lstlisting}[language=c, caption={Chromium UAR Vulnerability. This simple example would work for all possible tag values for arr1 }, captionpos=b, label={lst:chrome-uar-attack}]
void src_code(long delta, int val) {
    int* arr1 = malloc(64);
    int* arr2 = arr1;
    free(arr1);
    // arr2 is now a dangling pointer
    // increment the tag:
    arr2 += delta;
    // re-allocated memory:
    int* arr3 = malloc(64);
    // access re-allocated memory:
    arr2[0] = val;
}

src_code(0x40000000000000, val);
\end{lstlisting}
}
% simply incrementing the tag will make 0xF overflow into the next bit : Seg fault. So, need to change it to 0.

\paragraphb{Security} 
Due to the deterministic behavior at free (increment by one), 
an attacker can cause a use-after-free, with probability 1, by incrementing the tag of a dangling pointer by one.
Listing \ref{lst:chrome-uaf-attack} gives an example vulnerable code. 
The attacker uses pointer arithmetic to increment the tag of the dangling pointer {\tt arr2} by 1. Then, the pointer can be used to access freed memory.
Since the incremented tag is also re-used when re-allocating freed memory, an attacker could also cause a Use-after-realloc with an old dangling pointer, similar to Listing \ref{lst:chrome-uaf-attack}. 
%Table \ref{tab:survey-sec-summary} summarizes the detection probability of all other memory safety attacks.

\begin{lstlisting}[language=c, caption={Chromium use-after-free due to increment-by-1 tagging strategy.},captionpos=b, label={lst:chrome-uaf-attack}]
  void src_code(long delta, char val) {
      char* arr1 = malloc(64);
      char* arr2 = arr1;
      free(arr1);
      // arr2 is now a dangling pointer
      // increment the tag:
      arr2 += delta;
      // access freed memory:
      arr2[0] = val;
  }
  src_code(0x100000000000000, val);
\end{lstlisting}


% We list a simple example here, which would work for all tag values except 0xF, for which bit 60 will also be modified (certain code can still be attacked if the attacker can change the tag from 0xF to 0).
%Note that since free list pointers are stored in freed slots, the attacker can overwrite these pointers, and possibly their shadow pointers (to bypass corruption detection), if their encoding is not secure. This attack can be prevented by the heap scanning approach (~\cite{chrome-security-blog-uaf-scan}), only if the tag of the allocation was 0xf, since freed memory will not be quarantined otherwise.

%In terms of use-after-realloc, since the incremented tag is re-used for re-allocations, a benign UAR attack will be caught deterministically. But, a malicious attacker could access the newly allocated object with an old dangling pointer using their ability to increment its tag. This can be done similar to Listing \ref{lst:chrome-uaf-attack}.

\ignore{
Listing \ref{lst:chrome-uar-attack} shows example code on which this attack would work - we assume that {\tt arr3} re-uses the memory that was originally allocated to {\tt arr1}. The attacker can increment the dangling pointer {\tt arr2}'s tag, and can use it to access the new object. 
}

% tags +1 with dangling ptr: UAF, UAR, freelist ptr attack!!

\paragraphb{An Improvement} 
The increment-by-one strategy ensures that all 16 tags are used before the tag recycles to an old value.
A better way to do this is to choose a {\em random odd} 4-bit offset $\delta$ at startup and 
then have the {\tt free} function increment the tag by $\delta$ (mod 16).
This ensures that all 16 tags are used before the tag recycles, as before, but because the attacker does not know $\delta$,
it is harder to mount a use-after-free that succeeds with probability one. To further improve memory safety, the allocator could maintain a small array of {\em random odd} $\delta$s and the low-order bits of the starting address of the allocation could be used to determine which delta gets used when free-ing the allocation.

An alternative approach is to assign {\em random} tags at free, different from the current tag value. 
This will provide a similar security guarantee as the previous paragraph, but with a lower memory overhead.

==> eurosp2023-template/usage_survey_files/glibc.tex <==
\subsection{Glibc}
\label{sec:mte-impl-glibc}

Glibc, the GNU C Library, updated its implementation of the malloc and free functions to support ARM MTE for tagging heap memory \cite{glibc-mte-code, glibc-mte-allprs}. On every malloc and realloc, Glibc generates a new {\em random non-zero} tag using the {\sf IRG} instruction, 
and assigns it to all the granules in the allocated memory.  
It writes the tag in the top byte of the returned pointer.
On a call to {\tt free}, all the granules belonging to the freed allocation are tagged with~0.
This ensures that pointers to the freed space will no longer work.

% Also note that Rust internally uses glibc to manage memory.

% \begin{figure}[t]
% \centering
%  \includegraphics[width=0.37\textwidth]{figures/mte_glibc_tagging_diag.pdf}
% %  \vspace{-10pt}
%     \caption{glibc's tagging behavior. Allocation 1 and 2 are of size 64 \& 32 bytes respectively.}
% \label{fig:glibc-tagging}
% % \vspace{-10pt}
% \end{figure}

Glibc maintains an object's metadata in the 16 bytes preceding the start of the object, and that single granule is always tagged with tag value zero.
This metadata granule, which precedes every heap allocation, 
acts as a guard to prevent an overflow from one allocation to the next.

Lastly, Glibc checks for a double-free, by verifying that the tag in the provided pointer matches the tag of the memory being freed. 
Since the memory tag will be zero after being freed, the pointer's tag will not match on a double free.
% Figure \ref{fig:glibc-tagging} demonstrates this.
% % 0 at free | should random at free!!
% \begin{itemize}
%     \item malloc: Random tag is assigned to the memory, and to the returned pointer.
%     \item free: Freed memory is tagged with tag 0.
%     \item Internal Metadata tagged with 0. 
% \end{itemize}
%The Rust runtime internally uses glibc for memory management.

\smallskip
\paragraphb{Security}
We point out some weaknesses in this design.
We assume that the attacker has access to the application's source code and binary, 
and the attacker can craft heap pointers with arbitrary tags and addresses.
For simplicity, we assume that the source code of the system being attacked includes pointer arithmetic instructions
that let the attacker manipulate tags in pointers. 
In practice, this is often done using gadgets in the code that do the desired arithmetic.
%and overwriting function pointers or return addresses to call those gadgets.

\smallskip\noindent
Some attacks on Glibc's tagging strategy are possible due to the use of a deterministic tag, namely zero, 
for metadata and for freed space.

% has access to the address of one of the variables on the heap, which can be achieved by techniques such as heap spraying [TODO: maybe say using BROP? not sure if heap spraying can work against current systems with ASLR etc]. 
% We also assume that the attacker can craft pointers with arbitrary tags - this can be achieved easily by using pointer arithmetic to modify the top byte that contains the tag. We note that our threat model is similar to that used by~\cite{brop-hacking-blind}. 

% TODO: Mention can use ROP to gain both these capabilities, like BROP. Note that CFI based approaches make ROP harder but not impossible..?

\paragraphi{Overwriting the metadata} 
Since the attacker knows that metadata granules are always tagged with zero, 
they could use pointer arithmetic to change the tag of any object pointer to 0, and overwrite the metadata adjacent to the object. 
Listing~\ref{lst:glibc-md-attack-v2} gives a sample source code that is vulnerable to such an attack. The attacker iteratively subtracts one from {\tt arr1} pointer's tag until it becomes zero. Then, the attacker overwrites {\tt arr1}'s metadata at index -16 (16 bytes left from where {\tt arr1} starts). 
A key point is that this attack is guaranteed to work (with probability 1) because the metadata granule is always tagged with zero.  Such exploits can be chained with other vulnerabilities to gain root privilege or allow remote code execution~\cite{glibc-metadata-exploit-pz}.

% captionpos=b moves the caption to below the code listing.
 \begin{lstlisting}[language=c, caption={glibc Heap Tagging Metadata Vulnerability: The attacker controls the arguments ind, delta, val.}, captionpos=b, label={lst:glibc-md-attack-v2}]
  void src_code(int ind, long delta, char val) {
      char* arr1 = malloc(48);
      // change pointer tag to 0:
      while (((<long>(arr1) >> 56) % 16) > 0)
          arr1 -= delta;
      // overwrite metadata:
      arr1[ind] = val;
  }
  // overwrite arr1's metadata with val:
  src_code(-16, 0x100000000000000, val)
\end{lstlisting}
%       char* arr2 = malloc(32); NOT needed for metadata vulnerability.

\ignore{
Benign non-adjacent buffer overflows are probabilistically protected, i.e. they can only succeed with probability $1/16$ (since the memory granule being accessed could have any one of 15 non-zero tag values if allocated or 0 if free/metadata). Similarly, a malicious attacker attempting a non-adjacent overflow can only be successful with probability $1/16$, by trying to guess the memory tag.

% Non-adjacent
% This means that buffer overflows and user-after free / re-alloc bugs can be caught with 93.3\% probability (1 in 15 chance of random tag guess being correct).

 \begin{lstlisting}[language=c, caption=glibc Heap Tagging UAF Vulnerability,captionpos=b, label={lst:glibc-uaf-attack-v2}]
void src_code(long delta, int val) {
    char* arr1 = malloc(48);
    char* arr2 = arr1;
    free(arr1);
    // arr2 is now a dangling pointer
    // set tag to 0:
    while (((reinterpret_cast<long>(arr2) >> 56) % 16) > 0)
        arr2 -= delta;
    // overwrite freed memory:
    arr2[2] = val;
}

src_code(0x100000000000000, val);
\end{lstlisting}
}

\paragraphi{Use after free} 
Since Glibc changes the tags of freed memory to zero, an attacker can again use pointer arithmetic to modify a dangling pointer's tag to 0 and cause a use-after-free vulnerability. As before, the attack is guaranteed to work and can be done using code similar to Listing~\ref{lst:glibc-md-attack-v2}. 
The check for double-free can be similarly bypassed, by modifying the pointer tag to 0, which will then match the tag of freed memory.

Finally, consider a dangling pointer {\tt p} to a freed allocation.  
Once the space is reallocated to another buffer, there is a $1/15$ chance that the new tag will match the old tag (prior to the free).
If that happens then accessing memory using~{\tt p} will not trigger a tag mismatch exception
and enable a use-after-realloc.
The success probability is only $1/15$.
% Table \ref{tab:survey-sec-summary} summarizes the protection offered by the current {\tt glibc} implementation against other common memory unsafety attacks.

\ignore{
With respect to benign Use-after-realloc's, the library offers probabilistic protection since the tag of the old pointer could match the new memory tag assigned at re-allocation with probability $1/15$ (since a random tag is chosen from 15 possible non-zero tag values). Similarly, an attacker attempting a Use-after-realloc can succeed only with probability $1/15$ by trying to guess the new (non-zero) memory tag.

Lastly, uninitialized memory is zero-tagged and hence benign attempts to access it would be caught deterministically. But, a malicious attacker could access it by modifying a pointer's tag to 0 (similar to Listing~\ref{lst:glibc-uaf-attack-v2}).

We note that we only speculate that these attacks would work but have not actually run them, due to glibc compilation issues with QEMU.
% TODO: due to compilation issues?
}

\paragraphb{Improvements} 
A natural suggestion is to tag every metadata granule with a {\em random} tag that is different from the tag of the adjacent allocation to the right. 
This prevents the preceding allocation from overflowing into the adjacent allocation
because the overflow pointer cannot match both the tag of the metadata granule and the tag of the adjacent allocation.  
Moreover, it protects the metadata from an overflow from the preceding allocation with probability $15/16 \approx 93\%$.
It also ensures that a simple metadata attack, as in Listing~\ref{lst:glibc-md-attack-v2}, will not succeed with certainty;
it will succeed with probability at most $1/16$ because the attacker must correctly guess the tag of the metadata granule.

Similarly, freed memory could be tagged with a random tag that is different from its current tag value (instead of always tagging freed memory with zero).
As before, it prevents existing pointers from accessing freed memory and prevents a double free. 
More importantly, an attacker can no longer cause a use-after-free with certainty by setting the tag of a dangling pointer to zero.



==> eurosp2023-template/usage_survey_files/linux.tex <==
\subsection{Linux SLUB}
\label{sec:mte-impl-linux}

The Linux kernel uses three different slab-based memory allocators, SLUB, SLOB, and SLAB, with SLUB being the most widely used.
All three include support for software-based memory tagging using \href{https://www.kernel.org/doc/html/latest/dev-tools/kasan.html}{KASAN}.

The SLUB allocator was extended to support MTE, by adding a new hardware tag-based mode in \href{https://www.kernel.org/doc/html/latest/dev-tools/kasan.html}{KASAN} ~\cite{kasan-mte-code, linux-slub-tagging-ppt}.
It uses {\sf IRG} to generate a random tag value for a new memory allocation (via kmalloc), but excludes the tags 0xE and 0xF.
Hence, a new allocation is tagged with one of 14 tags. 
It sets this random tag as the tag for all the newly allocated granules and embeds the tag into the returned pointer. 
Since slab-based allocators round up the allocation size, they can allocate extra granules beyond the requested size. 
These granules are tagged with 0xE.
When memory is freed with a call to {\tt kfree}, all the freed granules are also assigned tag value 0xE. 
The tag 0xE is called the ``no access'' tag, although this ``no access'' property is not enforced by the hardware. 

For internal data structures, the allocator returns a pointer with the match-all tag (0xF) to speed-up memory allocation.
%This tag was selected to match the top byte 0xFF of native kernel pointers.
At startup, the kernel sets MTE's  % {\sf TCR\_EL1.TCMA1} 
flag to disable tag checking for pointers with a 0xF tag.
As a result, SLUB need not update the tags of the memory granules allocated for internal data structures, which speeds up memory allocation
but disables tag checking.
Note that no physical memory granule is ever tagged with the match-all tag 0xF.

The allocators implement explicit checks for double free: 
a call to free is rejected unless the pointer tag is either the match-all tag or it matches the current memory tag.
% the memory being freed is not already tagged with the invalid tag 0xE.

% \begin{itemize}
%     \item Random tag at malloc, invalid tag for freed and for extra memory allocated.
%     \item Match-all tag used for internal data structures.
% \end{itemize}

\paragraphb{Security} 
The allocator uses a {\em deterministic} tag (0xE) for freed space, and the same security concerns raised for Glibc with regard to user-after-free (and double-free) apply here as well.
% Table \ref{tab:survey-sec-summary} summarizes SLUB's protection against other common memory unsafety issues.

\ignore{
We use a threat model similar to what we described in \S\ref{sec:mte-impl-glibc}. We assume that the attacker has access to the kernel's source code (and version). For pointer crafting, we assume that there is a kernel API that does input-dependent pointer arithmetic, which can be called from user space. The attacker can hence call this API with specific inputs to craft a pointer with the desired tag and address.
% for analysing the security properties of hardware - based KASAN.

\paragraphi{Spatial Safety}
% TODO: malicious: adjacent: 
A malicious attacker could access the extra allocated granules (if any) adjacent to the allocation by updating the pointer's top byte to have a tag value of 0xE. Listing \ref{lst:linux-invalid-attack} demonstrates an example kernel API susceptible to such an attack. We assume that the allocation ends up in the 64-byte size class, and hence a total of 4 granules are allocated (1 extra granule). Note that, since the SLUB allocator does not tag any allocation's pointer with tag 0xE or 0xF, the arr1's tag is going to be less than 0xE. The attacker can increment the tag until is equal to 0xE, and then access the extra allocated granule.

But, an overflow attack into an adjacent allocation can only succeed with a 1 in 14 chance. Lastly, an attacker can overflow into a non-adjacent granule with a 1 in 15 chance (since the granule could be tagged with all values except 0xF).

% This means that overflow into this extra memory can be caught with 100\% probability, but non-adjacent overflows and user-after-frees can only be detected with 92.8\% probability (1 in 14 chance of random guess succeeding).

\begin{lstlisting}[language=c, caption={Linux SLUB Invalid tag Vulnerability. Here, we assume that our object lands in the 64-byte size class and hence 4 granules are allocated.}, captionpos=b, label={lst:linux-invalid-attack}]
void kernel_api(int ind, long delta, int val)
{
    int* arr1 = kmalloc(36);
    // set tag to 0xE:
    while (((reinterpret_cast<long>(arr1) >> 56) % 16) < 0xe)
        arr1 += delta;
    // access extra granule:
    arr1[ind] = val;
}

// attacker calls:
kernel_api(12, 0x40000000000000, val);
\end{lstlisting}

\begin{lstlisting}[language=c, caption=Linux SLUB UAF Vulnerability, captionpos=b, label={lst:linux-uaf-attack}]
void kernel_api(int ind, long delta, int val)
{
    int* arr1 = kmalloc(36);
    int* arr2 = arr1;
    // set tag to 0xE:
    while (((reinterpret_cast<long>(arr2) >> 56) % 16) < 0xe)
        arr2 += delta;
    // access free'd memory:
    free arr1;
    arr2[ind] = val;
}

// attacker calls:
kernel_api(0, 0x40000000000000, val);
\end{lstlisting}

\paragraphi{Temporal Safety} We use the same threat model as above, but with an added assumption that there is a dangling pointer. 

Because freed memory is tagged with 0xE value, hardware-based KASAN provides deterministic protection against benign use-after-frees, since a dangling pointer will not have this invalid tag. But, a malicious attacker could use pointer arithmetic to modify the dangling pointer's tag to 0 and then access freed memory. Listing \ref{lst:linux-uaf-attack} demonstrates an example kernel API that is vulnerable to this attack. With the ability to increment the dangling pointer's (arr2) tag to change it to 0xE, the attacker can access the freed memory, with ind value anywhere between 0 and 11 (since the allocation was of size 3 granules, fitting 12 integers).

Unintentional use-after-realloc's are protected probabilistically, i.e. the old pointer's tag (equal to the old allocation tag) might equal the new allocation's tag with a $1/14$ probability. Similarly, a malicious attacker attempting a use-after-realloc with an old pointer can only succeed with a $1/14$ chance by randomly guessing the new memory tag. 

\begin{lstlisting}[language=c, caption=Linux SLUB Match-all Vulnerability, captionpos=b, label={lst:linux-matchall-attack}]
void kernel_api(int ind,long delta,int val)
{
    int* arr1 = kmalloc(640);
    // set tag to 0xF:
    while (((reinterpret_cast<long>(arr1) >> 56) % 16) < 0xf)
        arr1 += delta;

    // access arbitrary memory:
    arr1[ind] = val;
}

// attacker calls:
kernel_api(100, 0x40000000000000, val);
\end{lstlisting}
}

\smallskip
\paragraphi{Exploiting the Match-all tag}
More importantly, there is an opportunity to exploit the match-all tag 0xF of MTE.  
Since Linux enables this match-all feature, any memory location on the kernel's heap can be accessed once a pointer with tag 0xF is crafted. 
An attacker can do so by using pointer arithmetic to modify the tag of any valid pointer to 0xF. 
This again can be done using code similar to Listing~\ref{lst:glibc-md-attack-v2}.
%Listing \ref{lst:linux-matchall-attack} demonstrates this an example kernel code that can be attacked like this - after changing the tag to 0xF, the attacker can access arbitrary indices (ind value). 
This diminishes the security provided by MTE since a single crafted pointer is enough to obtain read/write access to all kernel memory. 

%\paragraphb{Potential Improvements} It might be better to tag freed memory with another random tag value to protect against malicious use-after-free attacks, with probability ~93\% (i.e. $14/15$ if 0xF is excluded). Also, since the match-all tag allows accessing all memory with just one pointer crafting, it might be beneficial to update the KASAN implementation to disable the match-all feature.
% enabling the match-all tag feature of MTE, while simplifying implementation, can be exploited. it might be useful to update Linux' KASAN implementation so as not to use match-all pointers for internal metadata TODO

% Similar to the vulnerabilities in the glibc library, 
% tagging freed memory with a fixed tag can allow use-after-frees



==> eurosp2023-template/usage_survey_files/llvm_stack.tex <==
\subsection{LLVM Stack Tagging}
\label{sec:mte-impl-llvm}
LLVM, the backend used with clang, has been updated to assign MTE tags to stack variables in the function prologue~\cite{llvm-mte-stack-desc, llvm-mte-stack-code, scudo-heap-llvm-tagging-desc}. Similar to the Chrome allocator discussed in the previous section, LLVM uses an increment-by-one strategy to tag stack variables, which enables an overflow attack on stack variables that succeeds with probability one. We were able to successfully run this attack in an MTE-enabled VM in QEMU.
We discuss the implementation, the attack, and our suggested improvements in Appendix~\ref{sec:app-llvm}.

\ignore{
We use a similar threat model as used for analysing glibc.
% - the attacker has access to the application's source code and binary, and the attacker can craft stack pointers with arbitrary tags and addresses.

 \begin{lstlisting}[language=c, caption={LLVM Stack Tagging Vulnerability: The attacker controls the inputs ind, delta, val. This attack successfully ran on an MTE-enabled VM in QEMU for all possible tag values of {\tt arr2}.},captionpos=b, label={lst:llvm-spatial-attack}]
void src_code(int ind,long delta,int val) {
    int arr1 [12];
    int arr2 [8];
    // decrementing arr2's tag:
    int* a = arr2 - delta;
    // if 0, change tag to 1:
    if (<long>(a) <= 0xffffffffffffff )
        a += 15*delta;
    // access arr1 memory:
    a[ind] = val;
}

// overwrite arr1[2] with val:
src_code(10, 0x40000000000000, val)
\end{lstlisting}

\paragraphi{Spatial Safety} Since all objects in the same stack frame have different (but sequential) tags, benign overflows within the stack frame would be caught deterministically. But, a malicious attacker could cause an overflow into any other stack variable by incrementing the tag of a single pointer. Listing \ref{lst:llvm-spatial-attack} demonstrates an example vulnerable code - there are two buffers on the stack frame, and by decrementing {\tt arr2}'s tag by 1, the attacker can overflow into {\tt arr1}. We compiled this code using clang-11 and were able to successfully run this attack in an MTE-enabled VM in QEMU, for all possible tag values of {\tt arr2}.

We also successfully ran different versions of this attack wherein we a. change the tag of {\tt arr1} to 0 and overwrite the granule above the function's arguments, containing 0-tagged frame pointer and return address. This causes a segmentation fault in the program when exiting the function (this might be avoidable if stack canary/PAC~\cite{arm-pac-whitepaper} is used to protect return addresses), and b. we decrement the tag of {\tt arr1} to overwrite the function variables.
% , and c. increment {\tt arr2}'s tag to access the (uninitialized) granule below {\tt arr2}.

% A benign or malicious attempt to overwrite the return pointer can be detected based on other protections, e.g. stack canary or PAC. 
Lastly, overflowing into another stack frame can be caught probabilistically, since the pointer tag can match memory tag with only a 1 in 16 chance.


\paragraphb{Potential Improvements} While tagging the stack variables with incremental tags helps reduce register pressure, it does not protect against malicious overflows. It might be better to use a purely random tag for every variable in the stack frame. To lower register pressure, one could store only the tags in the registers instead of storing the tagged addresses - this might increase the performance overhead.

}

==> eurosp2023-template/usage_survey_files/scudo_android.tex <==
\subsection{Android Scudo}
\label{sec:mte-impl-scudo}
\href{https://llvm.org/docs/ScudoHardenedAllocator.html}{Scudo} is the default memory allocator used by the Android mobile OS. 
It uses two types of allocators:
a primary allocator for small-sized allocations,  and
a secondary allocator that manages large allocations (at least one page).
%, by using memory mapping primitives of the OS, e.g. mmap for Linux. 

% It supports MTE only for the primary allocator, and uses guard pages for the memory allocated by secondary allocator.
% TODO: sec alloca - guard pages and tag mem region bw start of mapping, start of alloca. Alloca still has tag 0

\subsubsection{The primary allocator} This is a size-class-based allocator, meaning that it has blocks of memory reserved for objects of specific sizes (also called size classes). Each block can have multiple chunks, with each chunk serving one allocation. It aligns allocations and metadata to 16 bytes, to support tagging granules. At malloc, a new random non-zero tag is generated, and all the allocated granules and the returned pointer are tagged with that value. Similarly, at free, a random non-zero tag is generated, and all the freed granules are tagged with it~\cite{scudo-heap-llvm-tagging-desc, scudo-mte-primary-code}. 
Note that this avoids deterministic tags for chunks. 
% It generates a new random non-zero tag on both malloc (tag assigned to memory granules and to the pointer) as well as free (tag assigned to freed memory granules) \cite{scudo-code}.

Interestingly the allocator implements the following optimization: when malloc re-allocates memory that was previously freed, and the new allocation has the same start address as the previous allocation, malloc re-uses the random tag (that was assigned at free) and assigns it to the pointer. 
If the new allocation is larger than the old one, it tags the additional granules with the same tag.
If the new allocation is smaller, it tags the granule at the very end of the new allocation with zero. 
This avoids the overhead of generating another tag and re-tagging all the granules.
%  TODO: 0 to adjacent granules?
%  Also, to protect adjacent buffer overflow with 100\% probability, it assigns random odd tags to the first, third, fifth (and so on) allocations, and random even tags to the 2nd, 4th, (and so on) allocations.

Scudo places 16 bytes of metadata (chunk header) in front of every allocation. This granule is tagged with zero,
% It tags its internal metadata (i.e. 16-byte chunk header in front of every allocation) with tag 0, 
but Scudo uses a 16-bit checksum to protect it, stored in the last two bytes of the header. 
The checksum is verified every time the header is accessed, to detect potential corruption.
This metadata granule acts as a guard to prevent a buffer overflow from the preceding allocation.

%Scudo uses the metadata to indicate whether a chunk is allocated or not -- it uses this flag to detect double free or invalid free calls. 
% Lastly, scudo can detect double free or invalid free calls by checking if the metadata 

Scudo provides additional features to enhance security. 
First, it tags the granule just following every allocation with zero. 
This acts as a guard to catch a buffer overflow emanating from the allocation.
The second feature is optional and controls how chunks are tagged. 
If turned on, Scudo generates odd tags for allocations in odd-numbered chunks and even tags for allocations in even-numbered chunks. 

\paragraphb{Security} %We use the same threat model as for Glibc.
The odd-even tagging feature protects against benign overflows on either side, since the allocations on either side would have a different parity tag. But, a malicious attacker could guess the tags of adjacent allocations with probability $1/8$, since the parity of an object gives away the parity of its adjacent objects in the same size class.

%Any other non-linear (non-adjacent) overflow is protected probabilistically with 93\% probability (1 in 16 chance of the pointer tag matching the memory tag), for both benign and malicious overflows.

\paragraphi{Temporal Safety} Since Scudo re-tags freed granules with a new random tag at free, any use-after-free attempt (benign or malicious) will be caught with probability $15/16 \approx 93\%$ if random tagging is used, and with $7/8 \approx 87\%$ probability if odd-even tagging is used. 
%
%The analysis is similar for benign use-after-realloc since Scudo re-uses the tag generated at free. 
More generally, the odd-even feature provides a security tradeoff: 
it ensures protection for a benign overflow into an adjacent allocation, 
but worsens the probability of catching a use-after-free and a benign use-after-realloc from $93\%$ to $87\%$.

Listing \ref{lst:scudo-uaf-attack} gives an example source code that is vulnerable to a use-after-free attack, 
caused by the optimization where Scudo re-uses the tag generated at free. 
The code first makes a big allocation {\tt a1}, which is then freed. 
Another allocation {\tt a2}, smaller than {\tt a1}, is made immediately, and if {\tt a2} is assigned to {\tt a1}'s freed memory, 
then the {\tt a2} pointer tag will match the tag of all the 40 freed granules. 
The allocator will re-tag the granule right next to {\tt a2} (the 31st granule) with zero, 
but an attacker can use {\tt a2} to overflow into granules 32 to 40 since they are not retagged.
% There is a possibility of an attack if a big allocation is made, followed by freeing it and making a smaller allocation, which lands at the same starting address as the original allocation. In this case, the new pointer (with tag equal to the one generated at free) can be used to access the additional granules in the old allocation, since they . Listing \ref{lst:scudo-uaf-attack} demonstrates this.

\noindent
\begin{minipage}[t]{.45\textwidth}
\begin{lstlisting}[language=c, caption={Scudo Use-after-free Vulnerability. The attack works for all values of ind between 496 and 639 (32nd to 40th granule).}, captionpos=b, label={lst:scudo-uaf-attack}]
  void src_code(int ind, char val)
  {
      char* a1 = malloc(640);
      free(a1);
      char* a2 = malloc(480);   // a2 == a1
      // overflow into a1's freed granules 
      arr2[ind] = val;
  }
  // attacker calls:
  src_code(500, val);
\end{lstlisting}
\end{minipage}
% ///
% This implies that an overflow from one chunk into any location in the preceding/succeding chunk will be caught with 100\% probability. 
% Note that non-adjacent overflow into random chunks can still succeed with 7-12\% probability based on parity.  
% But, this reduces use after free to 87\% probability (1 in 8 chance of random tag succeeding, since the parity of the chunk is known). This presents a spatial vs temporal safety trade-off.

% Overall, the tagging behavior in Scudo protects against spatial unsafety with 93-100\% and against temporal safety with 87-93\% probability, depending on the configuration of options listed above.

% TODO: when memory released to OS: tag data lost. [secondary alloc does free page to OS, primary can also do this]
\paragraphb{Potential Improvements} The use-after-free attack is possible because re-allocating a subset of freed memory does not re-tag the affected granules. To avoid this, it is important to generate a new random tag at malloc and use it to either tag the re-allocated granules or to tag the remaining free granules that remain free.

\subsubsection{Secondary Allocator} Since this allocator is only used for large allocations, Scudo does not tag allocated memory due to the large overhead of setting the tags for all the granules during malloc and free.
%We note that while there exist instructions to handle tag manipulation in blocks of 1 - 16 granules ({\sf LDGM, STGM}), they can only be used on Exception Level 1 (kernel) or higher. 
Instead, the allocator uses the following protections: it protects the allocation with a non-readable (using {\sc prot\_none}) guard page on the right.
The memory between the beginning of the page and the start of the allocation is tagged with a random non-zero tag.
This acts as a guard to prevent an overflow to the left, since all allocations are 0-tagged.
% MTE is used to tag the memory between the beginning of the page and the start of the allocation by tagging these granules with a random non-zero tag.
%- which acts as a redzone to catch linear overflows~\cite{scudo-secAllo-code}. 
To protect against temporal attacks, it sets freed pages as non-readable (using {\sc prot\_none}) to catch attempts to access freed memory~\cite{scudo-secAllo-code}.
% never re-uses the virtual addresses once these large allocations are freed. This is similar to how ASan puts freed addresses into quarantine~\cite{asan-atc-12} so as to detect usage of freed memory. Lastly, scudo also uses a copy-on-write reference page with a non-zero tag

\ignore{
\paragraphb{Security} 
\paragraphi{Spatial Safety} Since there are guard pages on the right of every allocation marked with {\sc prot\_none} (i.e. inaccessible memory), adjacent overflows will be caught deterministically. In terms of overflowing towards the left, a benign attempt will be caught deterministically since the memory on the left of every allocation is tagged with a non-zero tag, which will not match with the allocation's 0-tagged pointer. But a malicious attempt to overflow to the left could succeed with a 1 in 15 chance (if the attacker correctly guesses the non-zero tag). Non - adjacent overflows into other allocations will succeed since all allocations are tagged with 0.
% An attempt for adjacent overflow will be deterministically caught because of the guard pages, since they cannot be accessed a.
% Separate for Prim, Sec?

\paragraphi{Temporal Safety} Since freed memory is marked with {\sc prot\_none} (i.e. inaccessible memory), a use-after-free attempt, whether benign or malicious, will be caught deterministically. 

If memory is reallocated, then, a (0-tagged) dangling pointer would still be able to access the new object since it would also be tagged with zero.
% TODO: UAR? does scudo secondary allocator do re-allocation?


}

==> impl-weaknesses.tex <==
\section{Attacks on MTE Implementations}
In this section, we describe the weaknesses and potential spatial/temporal memory unsafety attacks on the implementations from the previous section.
%% Describe all the attack on the implementations from previous section.
TODO: Add benign vs malicious UAF/ Use after re-alloc. TODO: Add example codes for all attacks.

\paragraphb{Threat Model}
We assume that the attacker has access to the application's source code, and has access to the address of one of the variables on heap or on some function's stack frame, which can be achieved by techniques such as heap spraying [TODO: more examples]. Lastly, the attacker can craft pointers with arbitrary tags - this can be achieved easily by using pointer arithmetic to modify the top byte. Similar to Blind ROP's threat model.
% Based on the current implementations of memory tagging as listed above, there are many exploits possible if an attacker has the ability to craft a pointer, specifically being able to change the tag of a pointer. We list the potential exploits that we have identified:

\subsection{glibc} 
 
 \textbf{Spatial Safety Analysis}. Since there is metadata between every 2 allocations (each tagged with a random non-zero tag), which is tagged with 0, glibc deterministically protects against adjacent buffer overflows. Intuitively, the metadata acts as a redzone between allocations. But, non adjacent overflows can still succeed with 7\% probability (1 in 16 chance).
 
 \begin{lstlisting}[language=c, caption=glibc Heap Tagging UAF Vulnerability, label={lst:glibc-attack}]
void test(int ind) {
    int* arr1 = malloc(48);
    arr[0] = 13;
    int* arr2 = arr1;
    free(arr1);
    // arr2 is now a dangling pointer
    // set tag to 0:
    int* p = arr2 && (0xffffffffffffff);
    p[0] = 11;
}
\end{lstlisting}

 \begin{lstlisting}[language=c, caption=glibc Heap Tagging Metadata Vulnerability, label={lst:glibc-md-attack}]
void test(int ind) {
    int* arr1 = malloc(48);
    int* arr2 = arr1 - 1; // subtracts 4bytes
    // set tag to 0:
    arr2 = arr2 && (0xffffffffffffff);
}
\end{lstlisting}

\textbf{Temporal Safety Analysis}
As seen in \S\ref{sec:mte-impl-glibc}, glibc tags freed memory with 0. While this can protect against benign temporal attacks, (i.e. a developer unintentionally using a dangling pointer to access freed memory), it does not protect against a malicious attacker with access to a dangling pointer, attempting a user-after-free. The attacker can use pointer arithmetic to modify the dangling pointer's tag to 0, and then access the freed memory. Note that, glibc (and dlmalloc?) can use some freed chunks to store metadata, which is also tagged with 0 - hence allowing the attacker read/write access to this metadata as well. Listing \ref{lst:glibc-attack} lists the code demonstrating this.
%  it is possible to do use-after-free attacks with access to a dangling pointer, by modifying its tag to 0. 
TODO: double free?
 
 Lastly, since glibc tags all its internal metadata with tag 0, a malicious attacker can use pointer arithmetic to a. change the tag to 0, b. subtract 4 bytes to move the pointer to glibc's metadata (located just before any hep object). This can allow the attacker to have read/write access to the metadata.
%  one can alter the allocator's internal metadata, since glibc tags with tag 0 and is stored in the bytes preceding every allocation. 
Both of these exploits can be chained with other vulnerabilities to to get root privilege or allow code execution~\cite{glibc-metadata-exploit-pz}.

 TODO: glibc compilation issues with QEMU,  (does not compile in QEMU). As a result, we speculate that these attacks would work, but we have not actually run them.
% UAF and attacking metadata.
% Use after free (but not use after reallocation) is possible by changing the tag of a dangling pointer to 0. It might be possible to alter the allocator's metadata (also tagged with 0 tag) - which can be used for bigger exploits, e.g. getting root privilege ~\cite{glibc-metadata-exploit-pz}.

% Cross compiled glibc with memory tagging enabled.
% Enabled the memory tagging tunable. TODO
\paragraphb{Potential Improvements} It might be better to tag metadata as well as freed memory with a random tag. To still maintain deterministic protection against adjacent buffer overflows, glibc can enforce that the tags of metadata are different from the tags of adjacent allocations, by e.g. using odd tags for metadata and even tags for allocations.


\subsection{LLVM Stack Tagging} 
\begin{lstlisting}[language=c, caption=LLVM Stack Tagging Vulnerability, label={lst:llvm-attack}]
void test(int ind) {
    int arr1[12];
    int a = 100;
    test2(&a, ind);
}

void test2(int* ta, int ind) {
    // subtract tag in bits 59-56 by 1.
    int* ta_prev_tag = ta - (1<<54); 
    // overflowing into arr1
    ta_prev_ind[10] = 101;
}
\end{lstlisting}

LLVM tags successive allocations on a stack frame deterministically - i.e. uses consecutive tag values. This can protect against benign overflows, but if an attacker has access to a single variable in the stack frame, they can use pointer arithmetic to increment/decrement the tag and access all other variables in the same stack frame. Listing \ref{lst:llvm-attack} demonstrates this, wherein the function test calls function test2, and passes the address of its local variable a as an input. Then, in test2, the attacker can decrease the tag by 1 and get read/write access to the array arr1. It is not uncommon for functions to pass the address of their local variables to another function, example ..? QEMU: allocation\_tag\_mem calling address\_space\_translate. 
% Buffer overflow within a stack frame.
% It is possible to do adjacent Buffer overflow, since the tag of successive allocations on stack is deterministic. So, if an attacker knows the tag of one allocation (e.g. if function passes a variable to an attacker controlled function), and has the ability to craft a pointer, they can access all allocations in the function.

% Used Clang-11, cross compiled locally.



\paragraphb{Security Analysis \& Improvements} 
Attacks,

Add: We implemented the attack on a QEMU VM, and it works as expected.

Randomized Stack Tagging: Storing only tags in registers for local variables, instead of full tagged addresses. 

\subsection{Chromium} 
Since Chromium's PartitionAlloc simply increments the tag by 1 at free, and re-uses this tag at re-allocation, it can protect against benign Use-after-free and Use-after-reallocate attacks. But, a malicious attacker can easily exploit a dangling pointer, by using pointer arithmetic to increment the tag by 1 - allowing both Use-after-free and Use-after-reallocate attacks. 

ADD code snippet
% Use after free with a dangling pointer

\subsection{Linux SLUB} 
\begin{lstlisting}[language=c, caption=Linux SLUB Match-all Vulnerability, label={lst:linux-attack}]
void test(int ind) {
    int* arr1 = kmalloc(640);
    int* arr2 = arr1;
    // set tag to 0xF:
    arr2 = arr2 || (0x0f00000000000000);
    free(arr1);
    // set tag to 0xE: (UAF)
    arr2 = (arr2 && 0xffffffffffffff);
    arr2 = arr2 || 0x0e00000000000000;
}
\end{lstlisting}
Linux uses the tag value 0xE for freed memory and for extra memory at every allocation (due to rounding off the requested size). An attacker with access to a dangling pointer can hence change the tag to 0xE and do Use-after-free attack. Listing \ref{lst:linux-attack} shows this.

Since Linux memory allocator uses a match-all tag of 0xF for its internal metadata, any memory location can be accessed once a pointer with tag 0xF is crafted. An attacker can easily do so by creating a new heap variable and using pointer arithmetic to modify its tag value to 0xF (Listing \ref{lst:linux-attack} demonstrates this). This greatly diminishes the security provided by MTE - a single crafted pointer is enough to get read/write access to all kernel memory. 
% Also it is possible to read freed memory (use-after-free) and the extra allocated memory by crafting a pointer with the invalid tag, 0xE.





==> improvements.tex <==
\section{Strengthening MTE hardware}

\subsection{Tag Storage Compression}\label{sec:btree-storage}
\begin{itemize}
    \item MTE's security is limited since it uses only 4 bit tags to limit the memory overhead. 
    \item We can improve this security - memory tradeoff by compressing the tag storage
\end{itemize}

% We can improve this security - memory tradeoff by compressing the tag storage, which can allow using larger tags with same or lower memory overhead.

\subsubsection{Design}
\textbf{Data Structure}
We propose a run length encoding based B-Tree to save space, 
RLE: which is based on the idea of storing runs of data as a single data value and count, rather than as the original run, e.g. if there is a large memory allocation of size 512 bytes, then, rather than storing the same tag for 32 granules, we could just store the tag with the count and starting position of the run. 
We use B-Trees to store such runs, to allow for efficient inserts, updates and look-ups. We now explain our data structure based on RLE and B-Trees in more detail.

\begin{figure}
\includegraphics[]{figures/RLE_example.png}
\caption{\label{fig:rle-example} Run Length Encoding of a Tag array of size 16, with 4 different runs. The encoding involves storing the tag and the start position}
\end{figure}
%%  Explain our proposed improvements to save space in tagged memory, with the purpose of expanding the size of the tags.
% MTE's security is limited since it uses only 4 bit tags to limit the memory overhead. We can improve this security - memory tradeoff by compressing the tag storage. This can allow using larger tags with same or lower memory overhead. 

% We propose using run length encoding / btree - explain DS
%%  run-length encoding



\subsubsection{Theoretical Analysis}
% BTree mem formula
\begin{itemize}
    \item Define notation (runs, granules etc)
    \item Formula for \#runs a single node can store, space used by BTree in terms of \# runs.
    \item Space Savings relative to tag array formula
    \item Discuss 
\end{itemize}

% Relative space savings:
%   \begin{equation} \label{eq:single-chain-theory-period}
%      \frac{n}{g} * (1 + \frac{2* log(g) - 1}{t})
%  \end{equation} 

\subsubsection{Discussion}
\paragraphb{Per Page vs Global BTree}
% \textbf{Per Page BTree}
[TODO] Having a single B-Tree data structure for all of physical memory has the following disadvantages:
\begin{itemize}
    \item Algorithmic Complexity Attacks: An attacking process could make a lot of small allocations
    \item Multi threading : would require locking in global BTree
    \item Handling page swapping
\end{itemize}
Hence, We chose to implement a B-tree per page. 


\paragraphb{Dynamic Data Structure?} 
\begin{itemize}
    \item As the \# allocations within a page increases, it is possivle that the BTree might not fit within the tag array space (i.e. 128 bytes for a small page)
    \item We dynamically adapt our DS - switch to using a tag array if 
\end{itemize}
% \textbf{Dynamic?} There can be scenarios where the BTree can take more space than an array, if, for instance, a particular page had a large number of small memory allocations. To avoid this scenario, we dynamically adapt the data structure - if the number of allocations in a page exceeds a certain limit, we migrate the tag storage to an array for that page. Having a per page tag management allows us to make this decision at the page granularity.



\paragraphb{Cache Behavior/Locality} Compare b/w BTree and Tag Array.

TODO: Differences b/w theoretical and implementation numbers: a. Fragmentation, b. each node uses fixed 44bytes, and not based on \#keys!!!

% Tree based RLE compression, implemented in QEMU. 4-5 BTree, Modified ldg, stg, mte\_probe1 functions in QEMU to also use the BTree.

\subsubsection{Evaluation}
%% Experiments showing how our modifications affect the tagged memory size for common workloads, like Apache and other benchmarks.
\input{evaluation}

\subsection{A proposal for additional features}

%% Hardware support for invalid tag, to prevent use-after-free.

%% Stack tagging.

%% k-wise independence for tag generation

\subsubsection{H/W Supported Invalid Tags}  
Define 0 as invalid tags
\begin{itemize}
    \item Dont use it for any newly allocated memory
    \item Assign this to freed memory
    \item But if freed chunks storing metadata: use some other tag value
\end{itemize}
% We can extend Linux SLUB's invalid tag idea to hardware. If we could allow the user to define a particular tag as invalid (similar to how MTE allows using a match-all tag), it can provide a stronger security guarantee against use after free attacks, by assigning this invalid tag to freed memory. 
Provides deterministic protection against UAF attacks.

\subsubsection{k-wise Independent Tags}

\subsubsection{Randomized Stack Tagging} Storing only tags in registers for local variables.

\subsubsection{Storing Type information}. Since the BTree allows us to store tags in much smaller space, we can use larger tags, and also store type information within the tag.

==> mte-background.tex <==
\section{Overview of Memory Tagging}

%%  Describe what MTE does and how it works in detail.
%%  What is the purpose of MTE, how it is implemented in hardware, what the pointer structure looks like, etc.

Armv8.5 introduced Memory Tagging Extension (MTE) to improve memory safety of code written in unsafe languages without requiring source changes. It implements a simple lock-and-key based access to memory. Memory locations are tagged by adding a 4 bit metadata (called the tag or lock) to each 16 bytes of physical memory (called the Tag Granule). Pointers and virtual addresses are modified to contain the tag (i.e. key), in their top byte, using the Top Byte Ignore feature of Arm~\cite{arm-mte-blog}.

In this section we describe the operation of MTE.   
We fill in a number of important details that are not described in the
MTE whitepaper~\cite{arm-mte-blog}.

\paragraphb{Architectural Details} MTE adds a new memory type, Normal Tagged Memory to the architecture. Every load and store instruction is modified to compare the pointer's tag with the tag of the memory being accessed - generating an exception on tag mismatch, subject to system registers' configuration. 
% \footnote{The exception can be configured to be synchronous or asynchronous}. 

\paragraphb{Tag Checking Controls} MTE defines new system registers that allow controlling tag checks. For instance, the register TCO can be used to globally disable all memory tag checking. When it is enabled, there are two modes for handling tag mismatches - synchronous, which causes an exception and asynchronous, wherein the CPU accumulates tag check faults information in the TFSR\_EL1 system register. The kernel can then periodically check and report the faults asynchronously. [NOT periodic: The kernel detects the change during one of the following:
    - Context switching
    - Return to user/EL0
    - Kernel entry from EL1
    - Kernel exit to EL1 (summary: during context switch or switching between exception levels)
  - If the register has been updated by the PE the kernel clears it and
    reports the error.~\cite{linux-mte-async}]
The synchronous/asynchronous mode can be selected by each process, by calling prctl with the corresponding flag. The synchronous mode provides accurate information at the exception and better security guarantee but less performant than the asynchronous mode. It is recommended to use the asynchronous mode only for debugging.
% , whereas the asynchronous mode has better performance. [Todo: more detail on the tradeoff]

Lastly, the translation control register (TCR\_EL1) can be modified to use 0x1111 as a match-all tag, i.e. if TCMA bit is enabled, then all memory accesses (from EL1, i.e. kernel space) with pointer tag 0x1111 are unchecked. 

\paragraphb{ISA Extensions} 
The v8.5 ISA has new instructions for tag manipulation, 
% which can be used by compilers / memory allocators to manage memory tags.
% ADDG, SUBG instructions can be used to modify both the tag and the address separately by an immediate value.
which can be used by memory allocators (e.g. glibc) and by compilers (e.g. LLVM) to manage tagging when allocating / free-ing memory.

\paragraphi{Tag Generation} The instruction IRG can be used to generate a random tag. The user can also specify tag values to exclude using the GMI instruction, which modifies the GCR\_EL1 register.

\paragraphi{Memory Tag Manipulation} LDG/STG instructions have been added for getting/setting the tag for a single memory granule. STZG allows setting the tag along with zero-ing the memory. LDGM/STGM instructions allow bulk loads/stores for system use, which access tags for memory block of size specified by GMID\_EL1 register. Note that this register can only be accessed in EL1 (i.e. kernel mode).

\paragraphi{Tag \& Pointer Arithmetic} The ISA also includes ADDG/SUBG instructions, which are variants of ADD/SUB, intended for address arithmetic. They allow both the tag and the address to be separately modified with an immediate offset.
% \paragraphb{ARM MTE} 
% H/W implementation of memory tagging. Every time memory is allocated, a random 4-bit tag is chosen, and all the newly allocated memory granules (16 byte region of memory) as well as the address (pointer) are marked with this tag \footnote{The tag is stored in the unused bits in the pointer, since the only the low 48  bits are used for memory addressing}. The load and store instructions verify that the tag in the input pointer matches the memory tag, causing a hardware exception on mismatch.
% % ... Note that ARM ISA provides instructions such as IRG (generates random tag), LDG, STG (getting, setting memory tags), that can be used by the compiler / memory allocation libraries for tag management. Linux kernel has added support for tagged addresses .

% \subsection{Kernel changes}
% Linux kernel has added support for mem tagging, involving the following changes:

% \begin{itemize}
%     \item Tag management at clear, copy pages
%     \item Page level protection : PROT\_MTE \cite{linux-prot-mte}
%     \item Allowing tagged addresses - thread level \cite{linux-tag-addr-abi}
% \end{itemize}

\paragraphb{Tag Storage \& Caching} Tags are stored in a large array which is stored either in ECC (error correcting code memory) or in a part of RAM reserved by firmware at boot time. There is also a tag cache, used for pre-fetching tags when the cache lines are loaded for tagged memory.

\paragraphb{Page Swapping}

% \begin{itemize}
%     % \item Match all tags TCMA
%     \item Todo: Tag storage/caching
% \end{itemize}

\paragraphb{Linux Kernel Support} The Linux Kernel has been updated to support MTE. The prctl command can be used to a. enable tagged addresses for the calling thread, b. change the tag check fault behavior to synchronous / asynchronous, c. specify tags to be excluded by the IRG instruction ~\cite{linux-tag-addr-abi}. mprotect can be called with the flag PROT\_MTE for the pages that need to be protected with MTE~\cite{linux-mte-doc, linux-prot-mte}. By default, a process has tagged addressing and memory tag checking disabled - one needs to call prctl \& mprotect to enable MTE support. At fork, the new process inherits the parent's configuration, memory map attributes as well as the memory tags. 

Lastly, we note that kernel accesses to user memory are mostly not checked, and signal handlers are always called with tag checking disabled (by setting PSTATE.TCO to 0).

 TODO: Resetting tags of when a page is allocated to a process.

\subsection{Security Analysis}
We will now look into how well can MTE protect against different types of memory safety errors.

\paragraphb{Spatial Memory Safety} Attacks that involve overflowing into an adjacent or non-adjacent allocation, are protected with 93\% probability. This is because, there is always a 1 in 16 chance (there are only 16 unique tags) that the tag of the pointer will match the tag of the memory being accessed.

\paragraphb{Temporal Memory Safety} 

\subsection{Limitations}
While MTE is a promising low-overhead approach for memory safety, it does not protect against a. Intra-object buffer overflows~\cite{nss-intra-obj-bug} and b. Type confusion errors (we note that most type confusion bugs actually build upon spatial or temporal memory unsafety and hence will be probabilistically mitigated). It can be combined with other approaches such as \cite{eff-san} to protect against such attacks, but this is out-of-scope for our work. Todo: Side channel attacks could also be possible, e.g. based on Speculative execution~\cite{msrc-mte-secu-analy}

% TODO: 

\paragraphi{Blind - ROP Like Attacks} One could attack a server using MTE in a similar fashion as the Blind ROP attack~\cite{brop-hacking-blind} - determining the tag of a memory granule, by trying multiple guesses and checking if the server crashes and re-starts. But we note that this does not render MTE useless, since such an attack will only work if the server calls fork() to restart after a crash.

% \ignore{   %%%% move to related section at the end
% \subsection{Memory Safety}
% \begin{itemize}
%     \item Define
%     \item Spatial - Inter and Intra object overflows
%     \item Temporal - use after free
%     \item Type confusion
% \end{itemize}


% }


